Decomposition of Geometric Set Systems and Graphs

We study two decomposition problems in combinatorial geometry. The first part deals with the decomposition of multiple coverings of the plane. We say that a planar set is cover-decomposable if there is a constant m such that any m-fold covering of the plane with its translates is decomposable into two disjoint coverings of the whole plane. Pach conjectured that every convex set is cover-decomposable. We verify his conjecture for polygons. Moreover, if m is large enough, we prove that any m-fold covering can even be decomposed into k coverings. Then we show that the situation is exactly the opposite in 3 dimensions, for any polyhedron and any $m$ we construct an m-fold covering of the space that is not decomposable. We also give constructions that show that concave polygons are usually not cover-decomposable. We start the first part with a detailed survey of all results on the cover-decomposability of polygons. The second part investigates another geometric partition problem, related to planar representation of graphs. The slope number of a graph G is the smallest number s with the property that G has a straight-line drawing with edges of at most s distinct slopes and with no bends. We examine the slope number of bounded degree graphs. Our main results are that if the maximum degree is at least 5, then the slope number tends to infinity as the number of vertices grows but every graph with maximum degree at most 3 can be embedded with only five slopes. We also prove that such an embedding exists for the related notion called slope parameter. Finally, we study the planar slope number, defined only for planar graphs as the smallest number s with the property that the graph has a straight-line drawing in the plane without any crossings such that the edges are segments of only s distinct slopes. We show that the planar slope number of planar graphs with bounded degree is bounded.

==> bibbackup.tex <==
\bibitem[A10]{A10} B. \'Acs: S\'ikfed\'esek sz\'etbonthat\'os\'aga, Master Thesis.

\bibitem[A08]{A08} G. Aloupis, J. Cardinal, S. Collette, S. Langerman, D. Orden, P. Ramos: Decomposition of Multiple Coverings into More Parts, to appear in Discrete and Computational Geometry, arXiv:0807.0552v1.


\bibitem[ABH06]{AmBH} G.~Ambrus, J.~Bar\'at, and P.~Hajnal: The slope
    parameter of graphs, {\it Acta Sci.
    Math.~(Szeged)} {\bf 72}  (2006), no.~3-4, 875--889.

\bibitem[BMW06]{BMW06} J.~Bar\'at, J.~Matou\v sek, and D.~Wood: Bounded-degree
graphs have arbitrarily large geometric thickness, {\it Electronic
J. Combinatorics} {\bf 13}/1 (2006), R3.

\bibitem[BPR03]{BPR03} S.~Basu, R.~Pollack, and
M.-F.~Roy: {\em Algorithms in Real Algebraic Geometry},
Springer-Verlag, Berlin, 2003.

\bibitem[BC78]{BC78}
E.A.~Bender and E.R.~Canfield: The asymptotic number of
labeled graphs with given degree sequences, {\em J.
Combin. Theory Ser. A} {\bf 24} (1978), 296--307.

\bibitem[BK98]{BK98} T.~Biedl and G.~Kant: A better heuristic for orthogonal graph drawings, {\it Comput. Geom.} 9 (1998), pp. 159-180.

\bibitem[B07]{B07} A. L. Buchsbaum, A. Efrat, S. Jain, S. Venkatasubramanian and K. Yi: Restricted strip covering and the sensor cover problem, SODA 2007: 1056-1063.

\bibitem[BMP05]{BMP05}
P. Brass, J. Pach, and W. Moser: {\em Research Problems in
Discrete Geometry}, Springer, Berlin, 2005. 


%\bibitem{CS03} A Circle Packing Algorithm , by Chuck Collins and Kenneth Stephenson Computational Geometry: Theory and Applications, 25 (2003), pp. 233-256.


\bibitem[DETT99]{DETT99} G.~Di~Battista, P.~Eades, R.~Tamassia, and I.~G.~Tollis:
{\it Graph Drawing}, Prentice Hall, Upper Saddle River, N.J., 1999.

\bibitem[DEH00]{DiEH} M.~B.~Dillencourt, D.~Eppstein, and D.~S.~Hirschberg:
Geometric thickness of complete graphs, {\em J.~Graph Algorithms
Appl.} {\bf 4(3)} (2000), 5--17.

\bibitem[DESW07]{DESW07} V.~Dujmovi\'c, D.~Eppstein, M.~Suderman, and D.~R.~Wood:
Drawings of planar graphs with few slopes and segments,
{\em Comput. Geom.} {\bf 38} (2007), no. 3, 194--212.

\bibitem[DSW04]{DSW04}
V.~Dujmovi\'c, M.~Suderman, and D.R.~Wood: Really
straight graph drawings, in: {\em Graph Drawing (GD '04)}
(J.~Pach, ed.), {\em Lecture Notes in Computer Science}
{\bf 3383}, Springer-Verlag, Berlin, 2004, 122--132. 

\bibitem[DSW07]{DSW07} V.~Dujmovi\'c, M.~Suderman, and D.~R.~Wood:
Graph drawings with few slopes, {\em Comput. Geom.} {\bf 38} (2007), 181--193.

\bibitem[DW06]{DuW} V.~Dujmovi\'c and D.~R.~Wood: Graph treewidth and
geometric thickness parameters, in: {\em Proc.~13th Internat.~Symp.
on Graph Drawing (GD '05)} (P.~Healy and N.S.~Nikolov, eds.), {\em
Lecture Notes in Comput.~Sci.} {\bf 3843}, Springer, Berlin, 2006,
129--140.

\bibitem[DEK04]{DEK04} C.~A.~Duncan, D.~Eppstein, and S.~G.~Kobourov: The
geometric thickness of low degree graphs. In: {\it Proc. 20th ACM Symp.
on Computational Geometry (SoCG'04)}, ACM Press, 2004, 340--346.

\bibitem[EMS10]{EMS10} M. Elekes, T. Mátrai and L. Soukup: On splitting infinite-fold covers, to appear in Fund. Math.

\bibitem[E05]{En05} M.~Engelstein: Drawing graphs with few slopes,
Research paper submitted to the Intel Competition for high school
students, New York, October 2005.

\bibitem[E04]{E04} D.~Eppstein: Separating thickness from geometric
thickness, {\it Towards a Theory of Geometric Graphs (J.~Pach,
ed.), Contemporary Mathematics} {\bf 342}, Amer. Math. Soc,
Providence, 2004, 75--86.

\bibitem[E63]{E63} P. Erd\H os, On a combinatorial problem, Nordisk Mat. Tidskr. 11: 5-10.

\bibitem[EL75]{EL75} P. Erd\H os and L. Lov\'asz, Problems and results on 3-chromatic hypergraphs and some related questions, in A. Hajnal, R. Rado, and V. T. Sós, eds., Infinite and Finite Sets (to Paul Erdős on his 60th birthday). II. North-Holland. pp. 609-627.


\bibitem[F48]{F48} I. F\'ary, On straight line representation of planar graphs, {\em Acta Univ. Szeged. Sect. Sci. Math.} {\bf 11} (1948), 229--233.

\bibitem[FMR94]{FMR94} H.~de~Fraysseix, P.~O.~de~Mendez, P.~Rosenstiehl: On triangle contact graphs, {\em Combinatorics, Probability and Computing} {\bf 3} (1994), 233--246.

\bibitem[FPP89]{FPP89} H.~de~Fraysseix, J.~Pach, and R.~Pollack:
How to draw a planar graph on a grid, {\em Combinatorica} {\bf 10}(1) (1990), 41--51.

\bibitem[F10]{F10} R. Fulek, personal communication.

\bibitem[GV10]{GV10} M. Gibson and K. Varadarajan: Decomposing Coverings and the Planar Sensor Cover Problem, arXiv:0905.1093v1.


\bibitem[GT94]{GT94} A.~Garg and R.~Tamassia:
Planar drawings and angular resolution: Algorithms and bounds, {\em Second Annual European Symposium, Lecture Notes in Computer Science} {\bf 855}, Springer, 1994, 12--23.

\bibitem[HSV99]{HuSW} J.~P.~Hutchinson, T.~C.~Shermer, and A.~Vince: On
representations of some thickness-two graphs, {\em Comput.~Geom.}
{\bf 13} (1999), 161--171.

\bibitem[J86]{Ja} R.~E.~Jamison: Few slopes without collinearity, {\em
Discrete Math.} {\bf 60} (1986), 199--206.

\bibitem[JJ10]{JJ10} V. Jelinek, E. Jelinkov\'a, J. Kratochv\'{\i}l, B. Lidick\'y, M. Tesa\v r, and T. Vysko\v cil: The planar slope number of planar partial 3-trees of bounded degree. In: {\em Graph Drawing, Lecture Notes in Computer Science} {\bf 5849}, Springer, Berlin, 2010, 304--315.

\bibitem[K73]{Ka} P.~C.~Kainen: Thickness and coarseness of graphs, {\em
Abh.~Math.~Sem.~Univ.~Hamburg} {\bf 39} (1973), 88--95.

%\bibitem[K07]{K07} B. Keszegh: Weak Conflict-Free Colorings of Point Sets and
%Simple Regions, {\it Proc. Canadian Conference on Computational Geometry
%  (CCCG)} 2007, 97-100.

\bibitem[K36]{K36} P.~Koebe: Kontaktprobleme der konformen Abbildung,  {\em Berichte Verhand. Sächs. Akad. Wiss. Leipzig, Math.-Phys. Klasse} {\bf  88} (1936) 141--164.

\bibitem[KPP10]{KPP10} B.~Keszegh, J.~Pach and D.~Pálvölgyi: Drawing planar graphs of bounded degree with few slopes, in preparation.

\bibitem[KPPT10]{KPPT10} B.~Keszegh, J.~Pach, D.~Pálvölgyi, and G.~Tóth: Cubic graphs have bounded slope parameter, J. Graph Algorithms Appl. 14(1): 5-17 (2010).

\bibitem[KPPT08]{KPPT08} B.~Keszegh, J.~Pach, D.~Pálvölgyi, and G.~Tóth: Drawing cubic graphs with at most five slopes. {\em Comput. Geom.} {\bf 40} (2008), no. 2, 138--147.

\bibitem[LEC67]{LEC67} A.~Lempel, S.~Even, I.~Cederbaum: An algorithm for planarity testing of graphs, {\em Theory of Graphs} (P.~Rosenstiehl, ed.), Gordon and Breach, New York, 1967, 215--232 .

\bibitem[LMS91]{LMS91} Y.~Liu, A.~Morgana, B.~Simeone: General theoretical results on rectilinear embeddability of graphs, {\em Acta Math. Appl. Sinica} {\bf 7} (1991), 187--192.

\bibitem[MP94]{MP94} S.~Malitz and A.~Papakostas: On the angular resolution of planar graphs,  {\em SIAM J. Discrete Math.} {\bf  7} (1994), 172--183.

\bibitem[MP86]{MP86} P. Mani-Levitska, J. Pach: Decomposition problems for multiple coverings with unit balls, manuscript, 1986.

\bibitem[MSz07]{MSz07} P.~Mukkamala and M.~Szegedy: Geometric
    representation of cubic graphs with four directions,
    {\it Comput. Geom.} {\bf 42} (2009), 842--851.
    
\bibitem[MOS98]{MuOS} P.~Mutzel, T.~Odenthal, and M.~Scharbrodt: The
thickness of graphs: a survey, {\em Graphs Combin.} {\bf 14} (1998),
59--73.

\bibitem[P80]{P80} J. Pach:
Decomposition of multiple packing and covering,
Diskrete Geometrie, 2. Kolloq. Math. Inst. Univ. Salzburg, 169-178, 1980.

\bibitem[P86]{P86} J. Pach: Covering the plane with convex polygons,
{\it Discrete and Computational Geometry} {\bf 1} (1986), 73-81.

\bibitem[PP06]{PP06} J.~Pach and D.~P\'alv\"olgyi: Bounded-degree graphs can
have arbitrarily large slope numbers, {\it Electronic J.
Combinatorics} {\bf 13}/1 (2006), N1.

\bibitem[PPT10]{PPT10} J.~Pach, D.~Pálvölgyi, and G.~Tóth: Survey on the Decomposition of Multiple Coverings, in preparation.

\bibitem[PTT05]{PTT05} J. Pach, G. Tardos, G. T\'oth:
Indecomposable coverings,  In: The China--Japan Joint Conference on Discrete
Geometry, Combinatorics and Graph Theory (CJCDGCGT 2005), Lecture Notes in
Computer Science {\bf 4381}, Springer, Berlin, 2007.

\bibitem[PT06]{PT06} J.~Pach and G.~T\'oth: Crossing number of toroidal graphs,  {\em Graph drawing,   Lecture Notes in Comput. Sci.} {\bf 3843}, Springer, Berlin, 2006, 334--342.

\bibitem[PT07]{PT07} J. Pach, G. T\'oth:
Decomposition of multiple coverings into many parts,
in: {\it Proc. 23rd ACM Symposium on Computational Geometry, (SoCG07)} 2007,
133-137.
Also in: {\it Comput. Geom. Theory and Applications}, accepted.

\bibitem[P10]{P10} D. P\'alv\"olgyi:
Indecomposable coverings with concave polygons, to appear in Discrete and Computational Geometry.

\bibitem[PT10]{PT10} D. Pálvölgyi and G. Tóth: Convex polygons are cover-decomposable, Discrete and Computational Geometry 43(3): 483--496 (2010).

\bibitem[T09]{T09} G. Tardos, personal communication.

\bibitem[TT07]{TT07} G. Tardos, G. T\'oth:
Multiple coverings of the plane with triangles,
{\it Discrete and Computational Geometry} {\bf 38} (2007), 443-450.

\bibitem[U53]{U53} P.~Ungar: On diagrams representing maps, {\it J. London
Math. Soc.} {\bf 28} (1953), 336--342.

\bibitem[WC94]{WC94}
G.A.~Wade and J.-H.~Chu: Drawability of complete graphs
using a minimal slope set, {\em The Computer J.} {\bf
37}/2 (1994), 139--142.

==> concavefull.tex <==

This section is based on my paper, Indecomposable coverings with concave polygons.

A family of sets is a {\em $k$-fold} covering of a point set
%We call a covering of a point set in the plane by a family of sets {\em $k$-fold}
if every point is contained in at least $k$ of the sets. A covering is {\em decomposable} if the sets can be partitioned into two ($1$-fold) coverings. We say that a planar set is {\em cover-decomposable}, if there exists a $k$ such that every $k$-fold covering of the plane by its translates is decomposable. Pach \cite{P86} conjectured that all convex planar sets are cover-decomposable, this is still an open problem. The conjecture has been verified for open convex polygons in a series of papers. The main goal of this paper is to prove results about {\it not} cover-decomposable polygons. We start the introduction by an overview and end it with a summary of this paper.\\

The problem of decomposing coverings is closely related to the so-called \textit{sensor cover problem}. Here the problem is that if we are given an area that has to be monitored and a finite number of sensors, each of which can monitor a part of the given area and has a fixed amount of lifetime, then we have to come up with an optimal starting time for each sensor such that they together monitor the whole area for as long as possible (in this version, it is not allowed to switch on and off a sensor more than once). If every point is monitored by at least $k$ sensors, each of which has a battery that is good for one hour and we want to decide whether it is possible or not to monitor the whole area for two hours, then we get the decomposition problem. If we want to have longer coverage, we get a problem where we want to decompose into multiple coverings (not just two). It is another interesting problem when we allow to switch sensors on and off an arbitrary number of times, about this little is known. Our paper deals with the simplest version of the problem when we are trying to decompose into two coverings. For more on decomposition to multiple coverings see Aloupis et al. \cite{A08} and for results about the sensor cover problem, see Buchsbaum et al. \cite{B07}. A recent result of Gibson and Varadarajan \cite{GV10} gives a possible generalization of Theorem C. about decomposition to multiple coverings. First we give a summary of the previous results about decomposition of coverings with the translates of a polygon.

\medskip

\noindent {\bf Theorem A.} {Pach }\cite{P86} {\em Every centrally symmetric open convex polygon is cover-decomposable.}

\medskip

\noindent {\bf Theorem B.} {Tardos, Tóth }\cite{TT07} {\em Every open triangle is cover-decomposable.}

\medskip

\noindent {\bf Theorem C.} {P\'alv\"olgyi, Tóth }\cite{PT10} {\em Every open convex polygon is cover-decomposable.}

\medskip

In fact, a stronger statement was proved in the last paper. To understand this, we need another definition. So far our definition only concerned coverings of the {\it whole} plane, but we could investigate coverings of any fixed planar point set. We say that a planar set is {\it totally-cover-decomposable} if there is a $k$ such that any $k$-fold covering of {\it any} planar point set by its translates is decomposable. In earlier papers this property was not defined, however, the proofs all work for this stronger version. This is the first paper that makes distinction of these definitions. To avoid confusion, we will call the cover-decomposable sets in this paper {\em plane-cover-decomposable}. By definition, if a set is totally-cover-decomposable, then it is also plane-cover-decomposable. On the other hand, we cannot rule out the possibility that
there are sets, or even polygons, which are plane-cover-decomposable,
but not totally-cover-decomposable. %But, as we mentioned earlier, the previous theorems' proofs are all true for the strongest version, moreover, they even imply the following theorem.
%\begin{thm}\label{union} Every polygon, that is the union of a finite number of translates of the same open convex polygon, is totally-cover-decomposable (thus also plane-cover-decomposable).
%\end{thm}
%This is not a direct consequence of the earlier mentioned theorems but it can be derived easily from the proofs used in those papers. Before this paper, there was only one negative result about polygons.
From the negative direction very little is known.

\medskip

\noindent {\bf Theorem D.} {Pach, Tardos, Tóth }\cite{PTT05} {\em Concave quadrilaterals are not plane-cover-decomposable (thus neither totally-cover-decomposable).}

\medskip


The main result of this paper is a generalization of Theorem D. We show that {\em almost} all (open or closed) concave polygons are {\it not} totally-cover-decomposable and even suspect that they are not plane-cover-decomposable.

To state our result precisely, we need to define {\it wedges}.
Suppose we have two halflines, $e$ and $f$, both with a common endpoint $O$.
Then they divide the plane into two parts, $W_1$ $W_2$, which we call
{\em wedges}. A {\em closed wedge} contains its boundary, an {\em open wedge}
does not. Point $O$, where the two boundary lines meet, is called the {\em apex} of the
wedges. The {\em angle} of a wedge is the angle between its two boundary
halflines, measured inside the wedge. That is, the sum of the angles of $W_1$
and $W_2$ is $2\pi$.

We say that a pair of wedges is {\em special}, if\\
(i) there is a wedge of angle less than $\pi$ that contains both of the wedges,\\
(ii) none of the wedges contains the other wedge. (See Figure 1.)\\

\begin{figure}[ht]
\begin{center}
\scalebox{0.7}{\includegraphics{typespec.eps}}
%\hspace{2cm}
%\scalebox{0.6}{\includegraphics{typespec2.eps}}
\caption{Two possible pairs of special special wedges.}
\end{center}
\end{figure}

For any polygon, the neighborhood of each vertex can be extended to a wedge.
Those are called the {\em wedges of the polygon}.
Note that a convex polygon cannot have a special pair of wedges.
%Now we are ready to state the main result of this paper, which is proved in Section 2.
P\'alv\"olgyi and Tóth proved

\medskip

\noindent {\bf Theorem E.} {P\'alv\"olgyi, Tóth }\cite{PT10} {\em Every open polygon that has no special pair of wedges is totally-cover-decomposable.}

\medskip

Our main result is the following

\medskip

\noindent {\bf Theorem 1.} {\em If a polygon has a special pair of wedges, then it is not totally-cover-decomposable.}

\medskip

Together with the previous theorem, this gives a complete characterization
of totally-cover-de\-com\-posable open polygons; an open polygon is
totally-cover-decomposable if and only if it does not have a special pair of
wedges.

%This theorem and the results of \cite{PT} (see Lemma 8 in that paper) give a complete classification of open polygons with respect to totally-cover-decomposability.

%\begin{thm} An open polygon is totally-cover-decomposable if and only if it has no special pair of wedges. \end{thm}

We show that every concave polygon with no parallel sides
has a pair of special wedges, therefore we have

\medskip

\noindent {\bf Theorem 2.} {\em If a concave polygon has no parallel sides, then it is not totally-cover-decomposable.}

\medskip

The problem of deciding plane-cover-decomposability for concave polygons is still open. However, in Section 3, we prove that a large class of concave polygons are not plane-cover-decomposable. We also show that any ``interesting" covering of the plane uses only countably many translates. (However, we do not consider here the problem when every point is covered infinitely many times; the interested reader is referred to the recent paper of Elekes, M\'atrai and Soukup \cite{EMS10}.)\\

Finally, in Section 4, we investigate the problem in three or more dimensions. The notion of totally-cover-decomposability extends naturally and we can also introduce space-cover-decomposability. Previously, the following result was known.

\medskip

\noindent {\bf Theorem F.} {Mani-Levitska, Pach }\cite{MP86} {\em  The unit ball is not space-cover-decomposable.}

\medskip

Using our construction, we establish the first theorem for polytopes which shows that the higher  dimensional case is quite different from the two dimensional one.

\medskip

\noindent {\bf Theorem 3.} {\em No polytope is space-cover-decomposable.}

\medskip


\subsection{The Construction -- Proof of Theorems 1 and 2}

In this section, for any $k$ and any polygon $C$ that has a special pair of wedges, we present a (finite) point set and an indecomposable $k$-fold covering of it by (a finite number of) the translates of the polygon. We formulate (and solve) the problem in its dual form, like in \cite{P86} or \cite{TT07}. Fix $O$, the center of gravity of $C$ as our origin in the plane. For a planar set $S$ and a point $p$ in the plane we use $S(p)$ to denote the translate of $S$ by the vector $\vec{Op}$. Let $\bar{C}$ be the reflection through $O$ of $C$. For any point $x$, $x\in C(p_i)$ if and only if $p_i\in \bar{C}(x)$.
To see this, apply a reflection through the midpoint of the segment $xp_i$. This switches $C(p_i)$ and $\bar{C}(x)$, and also switches $p_i$ and $x$.

Consider any collection ${\cal C}=\{C(p_i)\ |\ i\in I\}$ of
translates of $C$ and a point set $X$. The collection ${\cal C}$ covers $x$ at least $k$ times if and only if
$\bar{C}(x)$ contains at least $k$ elements of the set
${P}=\{p_i\ |\ i\in I\}$. Therefore a $k$-fold covering of $X$ transforms into a point set such that for every $x \in X$ the set $\bar{C}(x)$ contains at least $k$ points of $P$.
The required decomposition of ${\cal C}$ exists if and only if
the set $P$ can be colored with two colors
such that every translate $\bar{C}(x)$ that contains at least $k$ elements
of $P$ contains at least one element of each color. Thus constructing a finite system of translates of $\bar{C}$ and a point set where this latter property fails is equivalent to constructing an indecomposable covering using the translates of $C$.

If $C$ has a special pair of wedges, then so does $\bar{C}$. We will use the following theorem to prove Theorem 1.

\begin{thm}\label{thm} For any pair of special wedges $V,W$ and for every $k,l$, there is a point set of cardinality ${k+l \choose k}-1$ such that for every coloring of $P$ with red and blue either there is a translate of $V$ containing $k$ red points and no blue points or there is a translate of $W$ containing $l$ blue points and no red points.
\end{thm}

\begin{proof}

%\noindent
%{\bf Proof of Theorem \ref{thm}.}\\
%\indent
Without loss of generality, suppose that the wedges are contained in the right halfplane.
%Using induction we will exhibit a set of points such that with any coloring either there is a translate of $V$ containing at least $k$ red points and no blue points or there is a translate of $W$ containing at least $l$ blue points and no red points. 

For $k=1$ the statement is trivial, just take $l$ points such that any one is contained alone in a translate of $W$. Similarly $k$ points will do for $l=1$. Let us suppose that we already have a counterexample for all $k'+l'<k+l$ and let us denote these by $P(k',l')$. The construction for $k$ and $l$ is the following.

Place a point $p$ in the plane and a suitable small scaled down copy of $P(k-1,l)$ left from $p$ such that any translate of $V$ with its apex in the neighborhood of $P(k-1,l)$ contains $p$, but none of the translates of $W$ with its apex in the neighborhood of $P(k-1,l)$ does. Similarly place $P(k,l-1)$ such that any translate of $W$ with its apex in the neighborhood of $P(k,l-1)$ contains $p$, but none of the translates of $V$ with its apex in the neighborhood of $P(k,l-1)$ does. (See Figure 2.)

\begin{figure}[ht]
\begin{center}
\scalebox{0.55}{\includegraphics{ellenpeldaindukcio.eps}}
\hspace{2cm}
\scalebox{0.65}{\includegraphics{ellenpeldajavitott.eps}}
\caption{Sketch of one step of the induction and the first few steps.}
\end{center}
\end{figure}

If $p$ is colored red, then\\
\indent
-- either the $P(k-1,l)$ part already contains a translate of $V$ that contains $k-1$ reds and no blues, and it contains $p$ as well, which gives together $k$ red points\\
\indent
-- or the $P(k-1,l)$ part contains a translate of $W$ that contains $l$ blues and no reds and it does not contain $p$.\\
\indent
The same reasoning works for the case when $p$ is colored blue.

Now we can calculate the number of points in $P(k,l)$. For $l=1$ and for $k=1$ we know that $|P(k,1)|=k$ and $|P(1,l)|=l$, while the induction gives $|P(k,l)|=1+|P(k-1,l)|+|P(k,l-1)|$. From this we have $|P(k,l)|={k+l \choose k}-1.$ %This completes the proof of Theorem \ref{thm}.\\
\end{proof}

It is easy to see that if we use this theorem for a pair of special wedges of $\bar{C}$ and $k=l$, then for every coloring of (a possibly scaled down copy of) the above point set with two colors there is a translate of $\bar{C}$ that contains at least $k$ points, but contains only one of the colors. This is because ``$\bar{C}$ can locally behave like any of its wedges''. Therefore this construction completes the proof of Theorem 1.\\

\noindent {\bf Remark.} We note that for $k=l$ the cardinality of the point set is approximately $4^{k}/\sqrt k$, this significantly improves the previously known construction of Pach, Tardos and Tóth \cite{PTT05} which used approximately $k^k$ points and worked only for quadrilaterals, and in general, for ``even more special" pairs of wedges (without giving the exact definition, see Figure 1/b). It can be proved that this exponential bound is close to optimal. Suppose that we have $n$ points and $n<2^{k-2}.$ Since there are two kinds of wedges, there are at most $2n$ essentially different translates that contain $k$ points. There are $2^n$ different colorings of the point set and each translate that contains $k$ points is monochromatic for $2^{n-k+1}$ of the colorings. Therefore, there are at most $2n2^{n-k+1}<2^n$ bad colorings, so there is a coloring with no monochromatic translates.
% because if there are $t$ kinds of wedges and $n<\frac{2^{k-1}}{t}$ points, then a good coloring always exists. This is true because there are less than $tn$ translates that contain exactly $k$ points, for each at most $(1/2)^{k-1}$ fraction of all the possible $2^n$ colorings are bad, therefore if we color the points randomly, then the chance of getting a monochromatic translate is less than $tn(1/2)^{k-1}<1$, thus there exists a good coloring.\\

Theorem 2 follows directly from the next result.

\begin{lem}\label{lem} Every concave polygon that has no parallel sides, has a special pair of wedges.
\end{lem}
%\noindent
%{\bf Proof of Lemma \ref{lem}.}\\
%\indent
\begin{proof}
Assume that the statement does not hold for a polygon $C$. There is a touching line $\ell$ to $C$ such that the intersection of $\ell$ and $C$ contains no segments and contains at least two vertices, $v_1$ and $v_2$. (Here we use that $C$ has no parallel sides.)
%of $C$ such that the intersection of the segment connecting them with $C$ is $\{v_1,v_2\}$.
Denote the wedges at $v_i$ by $W_i$. Is the pair $W_1,W_2$ special? They clearly fulfill the property (i), the only problem that can arise is that the translate of one of the wedges contains the other wedge. This means, without loss of generality, that the angle at $v_1$ contains the angle at $v_2$. Now let us take the two touching lines to $C$ that are parallel to the sides of $W_2$. It is impossible that both of these lines touch $v_2$, because then the touching line $\ell$ would touch only $v_2$ as well. Take a vertex $v_3$ from the touching line (or from one of these two lines) that does not touch $v_2$. (See Figure 3.) This cannot be $v_1$ because then the polygon would have two parallel sides. Is the pair $W_2,W_3$ special? They are contained in a halfplane (the one determined by the touching line). This means, again, that the angle at $v_2$ contains the angle at $v_3$. Now we can continue the reasoning with the touching lines to $C$ parallel to the sides of $W_3$, if they would both touch $v_3$, then the touching line $\ell$ would touch only $v_3$. This way we obtain the new vertices $v_4, v_5, \ldots$ what contradicts the fact the $C$ can have only a finite number of vertices. \end{proof}%This completes the proof of Lemma \ref{lem}.\\

\begin{figure}[ht]
\begin{center}
\scalebox{0.8}{\includegraphics{specialwedges.eps}}
\caption{How to find a special pair of wedges.}
\end{center}
\end{figure}

\subsection{Versions of cover-decomposability}

Here we consider different variants of cover-decomposability and prove relations between them.


\subsubsection{Number of sets: Finite, infinite or more}

We say that a set is {\em finite/countable-cover-decomposable}, if there exists a $k$ such that every $k$-fold covering of any point set by a finite/countable number of its translates is decomposable. 
So by definition we have: totally-cover-decomposable $\Rightarrow$ countable-cover-decomposable $\Rightarrow$ finite-cover-decomposable. But which of these implications can be reversed? We will prove that the first can be for ``nice'' sets.

It is well-known that the plane is hereditary Lindelöf, ie.\ if a point set is covered by open sets, then countably many of these sets also cover the point set. It is easy to see that the same holds for $k$-fold coverings as well. This observation implies the following lemma.

\begin{lem} An open set is totally-cover-decomposable if and only if it is countable-cover-decomposable.
\end{lem}

The same holds for ``nice'' closed sets, such as polygons or discs. We say that a closed set $C$ is {\em nice} if there is a $t$ and a set $\mathcal D$ of countably many closed halfdiscs such that if $t$ different translates of $C$ cover a point $p$, then their union covers a halfdisc from $\mathcal D$ centered at $p$ (meaning that $p$ is halving the straight side of the halfdisc) and the union of their interiors covers the interior of the halfdisc. For a polygon, $t$ can be the number of its vertices plus one, $\mathcal D$ can be the set of halfdiscs whose side is parallel to a side of the polygon and has rational length. For a disc, $t$ can be $2$ and $\mathcal D$ can be the set of halfdiscs whose side has a rational slope and a rational length. In fact every convex set is nice.

\begin{claim} Every closed convex set is nice.
\end{claim}
\begin{proof} Some parts of the boundary of the convex set $C$ might be segments, we call these sides. Trivially, every convex set can have only countably many sides. Choose $t=5$ and let the set of halfdiscs $\mathcal D$ be the ones whose side is either parallel to a side of $C$ or its slope is rational and has rational length. Assume that $5$ different translates of $C$ cover a point $p$. Shifting these translates back to $C$, denote the points that covered $p$ by $p_1, \ldots, p_5$. If any of these points is not on the boundary of $C$, we are done. The $p_1p_2p_3p_4p_5$ pentagon has two neighboring angles the sum of whose degrees is strictly bigger than $2\pi$, without loss of generality, $p_1$ and $p_2$. If $p_1p_2$ is also the side of $C$, then the $5$ translates cover a halfdisc whose side is parallel to $p_1p_2$, else they cover one whose side has a rational slope.
\end{proof}

Taking a rectangle verifies that $t=5$ is optimal in the previous proof.

\begin{lem} A nice set is totally-cover-decomposable if and only if it is infinite-cover-decomposable.
\end{lem}
\begin{proof} We have to show that if we have a covering of some point set $P$ by the translates of our nice, infinite-cover-decomposable set $C$, then we can suitably color the points of $P$. Denote by $P^*$ the points that are covered by $2$ copies of the same translate of the nice set $C$. Color one of these red, the other blue. Now we only have to deal with $P'=P\setminus P^*$ and we can suppose that there is only one copy of each translate. Now instead of coloring these translates, we rather show that we can choose countably many of them such that they still cover every point of $P'$ many times. Using after this that the set is infinite-cover-decomposable finishes the proof. So now we show that if there is a set of translates of $C$ that cover every point of $P'$ at least $kt$ times, then we can choose countably many of these translates that cover every point of $P'$ at least $k$ times. It is easy to see that it is enough if we show this for $k=1$ (since we can repeat this procedure $k$ times).

Denote the points that are contained in the interior of a translate by $P_0$. Because of the hereditary Lindelöf property, countably many translates cover $P_0$.
If a point $p\in P'$ is covered $t$ times, then because of the nice property of $C$, a halfdisc from $\mathcal D$ centered at $p$ is covered by these translates. We say that this (one of these) halfdisc(s) belongs to $p$. Take a partition of $P'\setminus P_0$ into countably many sets $P_1\cup P_2\cup\ldots$ such that the $i^{th}$ halfdisc belongs to the points of $P_i$. Now it is enough to show that $P_i$ can be covered by countably many translates. Denote the halfdisc belonging to the points of $P_i$ by $D_i$. Using the hereditary Lindelöf property for $P_i$ and open discs (not halfdiscs!) with the radius of $D_i$ centered at the points of $P_i$, we obtain a countable covering of $P_i$. Now replacing the open discs with closed halfdiscs still gives a covering of $P_i$ because otherwise we would have $p,q\in P_i$ such that $p$ is in the interior of $q+D_i$, but interior of $q+D_i$ is covered by the interiors of translates of $C$, which would imply $p\in P_0$, contradiction. Finally we can replace each of the halfdiscs belonging to the points of $P_i$ by $t$ translates of $C$, we are done.
\end{proof}

Unfortunately, we did not manage to establish any connection among finite- and countable-cover-decomposability. We conjecture that they are equivalent for nice sets (with a possible slight modification of the definition of nice).
If one manages to find such a statement, then it would imply that considering cover-decomposability, it does not matter whether the investigated geometric set is open or closed, as long as it is nice. For example, it is unknown whether closed triangles are cover-decomposable or not. We strongly believe that they are.

\subsubsection{Covering the whole plane}

%We say that a set is {\em plane-cover-decomposable}, if there exists a $k$ such that every $k$-fold covering of the plane by its translates is decomposable.
Remember that by definition if a set is totally-cover-decomposable, then it is also plane-cover-decomposable. However, the other direction is not always true. For example take the lower halfplane and ``attach'' to its top a pair of special wedges (see Figure 4). Then the counterexample using the special wedges works for a special point set, thus this set is not totally-cover-decomposable, but it is easy to see that a covering of the whole plane can always be decomposed.

For a given polygon $C$, our construction gives a set of points $S$ and a non-decomposable $k$-fold covering of $S$ by translates of $C$. It is not clear when we can extend this covering to a $k$-fold covering of the whole plane such that none of the new translates contain any point of $S$. This would be necessary to ensure that the covering remains non-decomposable.

%The problem is that the dual of our construction in Section 2 does not give a covering of the whole plane and it is not clear when it can be extended to one.

We show that in certain cases it can be extended, but it remains an open problem to decide whether plane- and totally-cover-decomposability are equivalent or not for open polygons/bounded sets. %Earlier Theorem D was known about quadrilaterals. We can generalize this theorem in the following form.

\begin{figure}[ht]
\begin{center}
\scalebox{0.77}{\includegraphics{halfplane.eps}}
\caption{The lower halfplane with a special pair of wedges at its top.}
\end{center}
\end{figure}

%\begin{thm}[Pach, Tardos, Tóth '05]\cite{PTT} No concave quadrilateral is plane-cover-decomposable.
%\end{thm}

\begin{thm}\label{plane} If a concave polygon $C$ has two special wedges that have a common locally touching line, and one of the two touching lines parallel to this line is touching $C$ in only a finite number of points (ie.\ does not contain a side), then it is not plane-cover-decomposable.
\end{thm}

\begin{proof} Assume, without loss of generality, that this locally touching line is vertical. We just have to extend our construction with the special wedges into a covering of the whole plane. Or, in the dual, we have to add more points to our construction such that every translate of $C$ will contain at least $k$ points. Of course, to preserve that the construction works, we cannot add more points into those translates that we used in the construction. Otherwise, our argument that the construction is correct, does not work. From the proof of the construction, we can see that the apices of the wedges all lay on the same vertical line. Therefore, the translates can all be obtained from each other via a vertical shift, because we had a vertical locally touching line to both wedges. Now we can simply add all points that are not contained in any of these original translates. Proving that every translate of $C$ contains at least $k$ points is equivalent to showing that the original translates do not cover any other translate of $C$. It is clear that they could only cover a translate that can be obtained from them via a vertical shift. On the touching vertical line each of the translates has only finitely many points. In the construction we have the freedom to perturbate the wedges a bit vertically, this way we can ensure that the intersection of each other translate (obtainable via a vertical shift) with this vertical line is not contained in the union of the original translates.
\end{proof}


\begin{figure}[ht]
\begin{center}
\scalebox{0.88}{\includegraphics{unknownpolygon.eps}}
\caption{A pentagon that is cover-decomposable but is not the union of a finite number of translates of the same convex polygon.}
\end{center}
\end{figure}


\begin{cor} A pentagon is totally-cover-decomposable if and only if it is plane-cover-decomposable.
\end{cor}
\begin{proof} All totally-cover-decomposable sets are also plane-cover-decomposable. (See an example on Figure 5.) If our pentagon is not totally-cover-decomposable, then it has a special pair of wedges and it must also have a touching line that touches it in these special wedges, thus we can use the previous theorem.
\end{proof} 


The same argument does not work for hexagons, for example we do not know whether the hexagon depicted in Figure 6/c is plane-cover-decomposable or not.% (but it is totally-cover-decomposable, the wedges determined by the angles at the vertices $A$ and $E$ give a special pair).
% because of the following example, hexagon $C$, that is depicted in Figure 5, because it has the following property.\\

\begin{figure}[ht]
\begin{center}
\scalebox{0.5}{\includegraphics{hatszogek.eps}}
%\hskip 2cm
%\scalebox{0.44}{\includegraphics{pcdk.eps}}
\caption{Three different polygons. (a): totally-cover-decomposable (hence, also plane-cover-decomposable),
(b): not plane-cover-decomposable, (hence neither totally-cover-decomposable),
(c): not totally-cover-decomposable, but not known if plane-cover-decomposable.}  %The polygon $C$ and its translates covering a dotted copy of it.}
\end{center}
\label{pcd}
\end{figure}

%{\em Self-Covering Property}: If we take three translates, $C_1, C_2$ and $C_3$, denoting the vertices of $C_i$ by $A_i, \ldots, G_i$, such that $A_1$, $A_2$ and $E_3$ are {\em very close} to each other, $A_2$ is to the right of $A_1$ and the slope of $A_1A_2$ is negative, then if we take a forth translate $C_4$, whose $x$-coordinate is the same as $C_1$'s and whose $y$-coordinate is the same as $C_2$'s, it will be covered by $C_1, C_2$ and $C_3$.\\ %Moreover, there is a $\delta$ such that if we intersect $C_4$ with an axis-parallel square of sidelength $\delta$, then this intersection will be covered by $one$ of $C_1, C_2$ or $C_3$.\\

%Indeed, observe that $C_4$ is covered almost entirely by $C_1$ and $C_2$, the only exception is the small vicinity of $B_4$, but that is covered by $C_3$ (see Figure 5).\\

\subsection{Higher Dimensions}
The situation is different for the space. For any polytope and any $k$, one can construct a $k$-fold covering of the space that is not decomposable. First note that it is enough to prove this result for the three dimensional space, since for higher dimensions we can simply intersect our polytope with a three dimensional space, use our construction for this three dimensional polytope and then extend it naturally. To prove the theorem for three dimensional polytopes, first we need some observations about polygons. Given two polygons and one side of each of them that are parallel to each other, we say that these sides are {\em directedly parallel} if the polygons are on the ``same side'' of the sides (ie.\ the halfplane which contains the first polygon and whose boundary contains this side of the first polygon can be shifted to contain the second polygon such that its boundary contains that side of the second polygon). We will slightly abuse this definition and say that a side is directedly parallel if it is directedly parallel to a side of the other polygon. We can similarly define {\em directedly parallel faces} for a single polytope. We say that a face is directedly parallel to another, if they are parallel to each other and the polytope is on the ``same side'' of the faces (eg.\ every face is directedly parallel to itself and if the polytope is convex, then to no other face).

\begin{lem}\label{bernadett} Given two convex polygons, both of which have at most two sides that are directedly parallel, there is always a special pair among their wedges.
\end{lem}
\begin{proof} Take the smallest wedge of the two polygons, excluding the ones that contain a wedge whose sides are both directedly parallel, if it exists. Without loss of generality, we can suppose that the right side of this minimal wedge is not directedly parallel and it is going to the right (ie.\ its direction is $(1,0)$), while the left side goes upwards. Take a wedge of the other polygon both of whose sides go upwards (there always must be one since the right side of the first wedge was not directedly parallel). If this second wedge is not contained in the first, we found a special pair. If the second wedge is contained in the first wedge, then because of the minimality of the first wedge, we get a contradiction.
\end{proof}

\smallskip
\noindent
{\bf Theorem 3.} {\em No polytope is space-cover-decomposable.}

%\begin{thm} No polyhedron is totally-cover-decomposable, not even space-cover-decomposable.
%\end{thm}
\begin{proof} We will, as usual, work in the dual case. This means that to prove that our polytope $C$ is not totally-cover-decomposable, we will exhibit a point set for any $k$ such that we cannot color it with two colors such that any translate of $C$ that contains at least $k$ points contains both colors. These points will be all in one plane, and the important translates of $C$ will intersect this plane either in a concave polygon or in one of two convex polygons. It is enough to show that this concave polygon is not cover-decomposable or that among the wedges of these convex polygons there is a special pair.\\Take a plane $\pi$ that is not parallel to any of the segments determined by the vertices of $C$. The touching planes of $C$ parallel to $\pi$ are touching $C$ in one vertex each, $A$ and $B$. Denote the planes parallel to $\pi$ that are very close to $A$ and $B$ and intersect $C$, by $\pi_A$ and $\pi_B$. Denote $C\cap \pi_A$ by $C_A$ and $C\cap \pi_B$ by $C_B$. Now we will have two cases.\\
\indent
{\bf Case 1.} $C_A$ or $C_B$ is concave.\\
Without loss of generality, assume $C_A$ is concave. Then since no two faces of $C$ incident to $A$ can be parallel to each other, with a perturbation of $\pi_A$ we can achieve that the sides of $C_A$ are not parallel. After this, using Theorem 2, we are done.\\\indent
{\bf Case 2.} Both $C_A$ and $C_B$ are convex.\\
Now by perturbing $\pi$, we cannot necessarily achieve that $C_A$ and $C_B$ have no parallel sides, but we can achieve that they have at most two directedly parallel sides. This is true because there can be at most two pairs of faces that are directedly parallel to each other and one of them is incident to $A$, the other to $B$, %(the definition is analogous to the definition of parallel sides), 
since $A$ is touched from above, $B$ from below by the plane parallel to $\pi$. Therefore $C_A$ and $C_B$ satisfy the conditions of Lemma 4.1, this finishes the proof of totally-cover-decomposability.

To prove space-cover-decomposability, just as in  the proof of Theorem \ref{plane}, we have to add more points to the constructions, such that every translate will contain at least $k$ points, but we do not add any points to the original translates of our construction. This is the same as showing that these original translates do not cover any other translate. Note that there are two types of original translates (depending on which wedge of it we use) and translates of the same type can be obtained from each other via a shift that is parallel to the side of the halfplane in $\pi$ that contains our special wedges. This means that the centers of all the original translates lay in one plane. With a little perturbation of the construction, we can achieve that this plane is in general position with respect to the polytope. But in this case it is clear that the translates used in our construction cannot cover any other translate, this proves space-cover-decomposability.
\end{proof}

\subsection{Concluding Remarks and Acknowledgement}

A lot of questions remain open. In three dimensions neither polytopes, nor unit balls are cover-decomposable. Is there any nice (eg.\ open and bounded) set in three dimensions that is cover-de\-com\-posable? Maybe such nice sets only exist in the plane.

In the first part of Section 2, we have seen that interesting covers with translates of nice sets only use countably many translates. We could not prove, but conjecture, that every cover can be somehow reduced to a locally finite cover. Is it true that if a nice set is finite-cover-decomposable, then it is also countable-cover-decomposable? This would have implications about the cover-decomposability of closed sets. Are closed, convex polygons cover-decomposable?

In the second part of Section 3, we have seen that our construction is not naturally extendable to give an indecomposable covering of the whole plane, maybe the reason for this is that it is impossible to find such a covering. Are there polygons that are not totally-cover-decomposable but plane-cover-decomposable?\\

I would like to thank G\'eza T\'oth for uncountably many discussions, ideas and suggestions with which he contributed to this paper incredibly much. I would also like to express my gratitude to G\'abor Tardos and J\'anos Pach for their observations and advice. I would also like to thank the referees for their several useful comments and Bernadett \'Acs for calling my attention to the incompleteness of the original proof of Lemma \ref{bernadett}.

==> convexfull.tex <==

This section is based on our paper with G\'eza T\'oth, Convex polygons are cover-decomposable.

Our main result is Theorem A. (iii), restated as

\medskip

\noindent {\bf Theorem 1.} {\em Every open convex polygon
is cover-decomposable.}

\medskip


Just like in \cite{P86} and in \cite{TT07}, we formulate
and solve the problem in its dual
form.
That is, suppose $P$ is a polygon of $n$ vertices and
we have a collection
${\cal P}=\{\ P_i\ |\ i\in I\ \}$ of translates of $P$.
Let $O_i$ be the center of gravity of $P_i$.
The collection ${\cal P}$ is a $k$-fold covering of the plane
if and only if every translate of $\bar{P}$, the reflection of $P$ through the
origin, contains at least $k$ points of the collection
${\cal O}=\{\ O_i\ |\ i\in I\ \}$.

The collection ${\cal P}=\{\ P_i\ |\ i\in I\ \}$ can be decomposed into two
coverings
if and only if the set ${\cal O}=\{\ O_i\ |\ i\in I\ \}$ can be colored with
two colors, such that  every translate of $\bar{P}$ contains a point of both
colors.

Divide the plane into small regions, say, squares, such that
each square contains at most one vertex of
any translate
of $\bar{P}$. If a translate of $\bar{P}$
contains sufficiently many points of ${\cal O}$, then it contains many
points of ${\cal O}$ in one of the little squares.
We color the points of
${\cal O}$ separately in each of the squares.
If we concentrate
on points in just one of the little squares, then instead of translates of
$\bar{P}$ we can consider translates of $n$ different wedges,
corresponding to the $n$ vertices of $P$.

In Section 2 we prove some results about coloring point sets with respect to
translates of wedges. In Section 3 we formulate the problem precisely
in the dual version, and apply the results of Section 2 to prove Theorem 1.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Preparation}

Suppose we have two halflines, $e$ and $f$, both of endpoint $O$.
Then they divide the plane into two parts, $W_1$ $W_2$, which we call
{\em wedges}. A {\em closed wedge} contains its boundary, an {\em open wedge}
does not. Point $O$, where the two boundary lines meet, is called the {\em apex} of the
wedges. The {\em angle} of a wedge is the angle between its two boundary
halflines, measured inside the wedge. That is, the sum of the angles of $W_1$
and $W_2$ is $2\pi$.
Now let $W$ be a wedge, and $X$ be a point in the plane. A translate of $W$
such that its apex is at $X$, is denoted by $W(X)$.
More generally, for points $X_1, X_2, \ldots X_k$,
$W(X_1, X_2, \ldots X_k)$ denotes the {\em minimal} translate of $W$
(for containment) whose
closure
contains $X_1, X_2, \ldots X_k$.
The set of all translates
of $W$ is denoted by $Tr^W$.
Let $-W$ denote the reflection of $W$ about the origin.

\medskip

\noindent {\bf Definition 1.}
Suppose that ${\cal W}=\{\ W_i\ |\ i\in I\ \}$ is a collection of wedges.
$\cal W$ is said to be {\em non-conflicting} or simply NC, if there is a
constant $k$ with the
following property.
Any finite set of points $S$ can be colored with two colors such that
any translate of a wedge $W\in {\cal W}$ that contains at least $k$ points of
$S$, contains a point of both colors. 
%This was investigated for other sets by Keszegh \cite{K07}.

\medskip

For any fixed  ${\cal W}$ and $S$, we can and will
assume without loss of generality
that the points of $S$ are in general position with respect to $\cal W$, that
is, they do not determine a line parallel to the boundary line of any
$W\in {\cal W}$.
Indeed, if there are two such points, 
slightly perturb the points.

It is easy to see that every subset of the original point set 
that can be cut off by a translate of a $W\in {\cal W}$, 
can also be cut off the perturbed point set. 

First suppose that we have only one open wedge, that is, ${\cal W}=\{ W\}$.

\medskip

\noindent {\bf Lemma 1.} {\em A single wedge is NC.}

\medskip

\noindent {\bf Proof of Lemma 1.}
Let $S$ be a finite point set and $W$ a wedge. 
We prove the statement with $k=3$, that is, 
$S$ can be colored with two colors such that
any translate of $W$ that contains at least $3$ points of
$S$, contains a point of both colors. 
Suppose first that the angle of $W$ is at least $\pi$. Then $W$ is the union
of two halfplanes, $A$ and $B$.
Take the translate of $A$ (resp. $B$) that contains exactly two points of $S$,
say,
$A_1$ and $A_2$ (resp. $B_1$ and $B_2$).
There might be coincidences between $A_1$, $A_2$ and $B_1$, $B_2$,
therefore the set $\{ A_1, A_2, B_1, B_2 \}$ contains two, three, or four
different points. But in any case, we can color $\{ A_1, A_2, B_1, B_2 \}$
such that $A_1$ and $A_2$ (resp. $B_1$ and $B_2$) are of different colors.
Now, if a translate of $W$ contains three points, it contains either
$A_1$ and $A_2$, or $B_1$ and $B_2$, and we are done.

\smallskip

Suppose now that the angle of $W$ is less than $\pi$. We give two proofs in
this case, since we will apply the ideas of both proofs later.
In fact, we show that in this case the NC property holds with $k=2$. 
We can assume that the positive $x$-axis is in $W$, and that no two points
have the same $y$-coordinate.
Both of these can be achieved by an appropriate rotation.
We say that $X<_yY$ if the $y$-coordinate of $X$ is smaller than the
$y$-coordinate of $Y$. This ordering is called the $y$-ordering.
A subset $I$ of $S$ is an {\em interval} of $S$
if $\forall X<_y Y<_y Z\in S: X,Z\in I \rightarrow Y\in I.$

The {\em boundary} of $S$ with respect to $W$,
$Bd^W(S)=\{X\in P:W(X)\cap S=\emptyset\}.$
Note that a translate of $W$ always intersects the boundary in an interval.
For each $X\in Bd^W(S)$ the {\em shadow} of $X$ is
$Sh^W(X)=\{Y\in S: W(Y)\cap Bd^W(S)=X\}.$
Observe that $\forall X,Y\in Bd^W(S): Sh^W(X)\cap Sh^W(Y)=\emptyset.$

For the first proof, color the points of the boundary alternating, according to the order $<_y$.
For every boundary point $X$,
color every point in the shadow of $X$ to the other color than $X$.
Color the rest of the points arbitrarily.
Any translate of $W$ that contains at least two points,
contains one or two boundary points.
If it contains one boundary point, then the other point is in its shadow,
so they have different colors.
If it contains two boundary points, then they are consecutive points according
to the $y$-order, so they have different colors again.
This finishes the first proof.
%Later we will refer to this coloring as {\em boundary-alternating}
%coloring with respect to $W$.

\begin{figure}[htb]
\begin{center}
\scalebox{0.4}{\includegraphics{replace.eps}}
\caption{$Z$ replaces $X$ in $W(2; y)$.}
\end{center}
\end{figure}

For the second proof,
for any fixed $y$, let $W(2;y)$ be the translate of $W$
which (1) contains at most two points of $S$, (2) its apex has $y$-coordinate
$y$, and (3) its apex has minimal $x$-coordinate.
It is easy to see that for any $y$, $W(2;y)$ is uniquely defined.
Examine, how $W(2;y)$ changes as $y$ runs over the real numbers.
If $y$ is very small (smaller than the $y$-coordinate of the points of $S$),
then  $W(2;y)$ contains two points, say $X$ and $Y$, and one more on its boundary.
As we increase $y$, the apex of $W(2;y)$ changes continuously.
How can the set $\{ X, Y\}$, of the two points in $W(2;y)$ change?
For a certain value of $y$, one of them, say, $X$, moves to the boundary. At
this point we have $Y$ inside, and two points, $X$, and $Z$ on the boundary.
If we slightly further increase $y$, then $Z$ {\em replaces} $X$, that is,
$Y$ and $Z$ will be in $W(2;y)$ (see Figure 1). As $y$ increases to infinity,
the set $\{ Z, Y\}$, could change several times, but the same way.
Define a graph whose vertices are the points of $S$, and two vertices, $U$ and
$V$ are connected iff $V$ replaced $U$ during the procedure.
We get two paths, $P_1$ and $P_2$. The pair $(P_1, P_2)$ is called
the {\em path decomposition of $S$ with respect to $W$, of order two}.

On Figure 2, two examples are given. 
The vertices of $P_1$ are $X_1, X_2, \ldots $, and the 
vertices of $P_2$ are $Y_1, Y_2, \ldots $.
On both examples, the translates of $W$ are given in the positions when 
some point is replacing another.

Color the vertices of $P_1$ red, the vertices of $P_2$ blue.
Observe that each translate of $W$ that
contains at least two points, contains at least one vertex of both $P_1$ and
$P_2$. This completes the second proof. \hfill $\Box$



\begin{figure}[htb]
\begin{center}
\scalebox{0.8}{\includegraphics{path1.eps}}
\caption{Path decompositions of order two. $P_1=X_1X_2\ldots $,
  $P_2=Y_1Y_2\ldots $.}
%The points of the two paths are denoted by $X$ and $Y$. 
%On the left figure, we have given the wedges that contain exactly 
%two points, while on the right, the moment of one point replacing another is illustrated.
\end{center}
\end{figure}

\smallskip

Now we can turn to the case when we have
translates of {\em two} wedges at the same time.
We distinguish several cases according to the relative
position of the two wedges, $V$ and $W$.

\smallskip

{\bf Type 1 (Big):} One of the wedges has angle at least $\pi$.

\smallskip

For the other cases, we can assume without loss of generality that
$W$ contains the positive $x$-axis.
% and is symmetric on it.
Extend the boundary halflines of $W$ to lines, they divide the plane
into four parts, Upper, Lower, Left, and Right, which is $W$ itself.
See Figure 3.


\begin{figure}[htb]
\begin{center}
\scalebox{0.4}{\includegraphics{w.eps}}
\caption{Wedge $W$}
\end{center}
\end{figure}
%

\smallskip

{\bf Type 2 (Halfplane):} One side of $V$ is in Right and the other one is in
Left. That is, the union of the wedges cover a halfplane. See Figure 4.

\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{t2.eps}}
\caption{Type 2 (Halfplane)}
\end{center}
\end{figure}
%


\smallskip

{\bf Type 3 (Contain):}
Either (i) one side of $V$ is in Upper, the other one is in Lower, or
(ii) both sides are in Right or (iii) both sides are in Left. See Figure 5. 

\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{t3.eps}}
\caption{Type 3 (Contain)}
\end{center}
\end{figure}
%


\smallskip

{\bf Type 4. (Hard):} One side of $V$ is in Left and the other one is in Upper or
Lower.
This will be the hardest case. See Figure 6. 

\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{t4.eps}}
\caption{Type 4 (Hard)}
\end{center}
\end{figure}
%


\smallskip

{\bf Type 5. (Special):} Either (i)
one side of $V$ is in Right and the other one is in Upper or Lower,
or (ii) both sides are in Upper, or (iii) both sides are in Lower.
That is, the union of the wedges is in an open
halfplane whose boundary contains the origin, but
none of them contain the other. See Figure 7. 



\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{t5.eps}}
\caption{Type 5 (Special)}
\end{center}
\end{figure}
%


\smallskip

It is not hard to see that there are no other possibilities.
Observe that two wedges corresponding to the vertices 
of a convex polygon cannot be of type 1 (Big) or of type 5 (Special).
This will be used in the proof of Theorem 1. 


It is shown in \cite{P10} that if ${\cal W}=\{ V, W\}$ is a set of two wedges
of type 5 (Special), then $\cal W$ is {\em not} NC. In a series of Lemmas we show that all
other pairs are NC.

\medskip


\noindent {\bf Lemma 2.} {\em Let ${\cal W}=\{ V, W\}$ be
a set of two wedges, of type 3 (Contain).
Then $\cal W$ is NC.}

\medskip

Suppose that $U$ is a wedge that contains the positive $x$-axis and has angle
less than $\pi$. For any $k>0$, and point set $S$, let $Tr^U_k(S)$ be the set
of translates of $U$ that contain exactly $k$ points of $S$.

Just like in the proof of Lemma 1,
for any fixed $y$, and $k>0$,
let $U(k;y)$ be the translate of $U$
which (1) contains at most $k$ points of $S$, (2) its apex has $y$-coordinate
$y$, and (3) its apex has minimal $x$-coordinate.
If $y$ is very small,
then  $U(k;y)$ contains $k$ points, say $X_1, X_2, \ldots, X_k$,
and one more on its boundary.
As we increase $y$, the apex of $U(k;y)$ changes continuously.
For a certain value of $y$, one of $X_1, X_2, \ldots, X_k$,
say, $X_1$, moves to the boundary. At
this point we have $X_2, \ldots, X_k$ inside,
and two points, $X_1$, and $X_1'$ on the boundary.
If we slightly further increase $y$, then $X_1'$ {\em replaces} $X_1$, that
is, $X_1'$ and $X_2, \ldots, X_k$
will be in $U(k;y)$. As $y$ increases to infinity,
some other points could be replaced similarly.
Define a graph whose vertices are the points of $S$, and two vertices, $X$ and
$Y$ are connected iff $X$ replaced $Y$ during the procedure.
We get $k$ paths, $P^U_1, P^U_2, \ldots, P^U_k$.
Each translate of $U$ that
contains at least $k$ points of $S$,
contains at least one vertex of each of
$P^U_1, P^U_2, \ldots, P^U_k$.
The $k$-tuple $(P^U_1, P^U_2, \ldots, P^U_k)$ is called
the {\em path decomposition of $S$ with respect to $W$, of order $k$}.



\medskip


\noindent {\bf Proof of Lemma 2.}
We can assume that $W\supset V$ or  $W\supset -V$
and $W$ contains the positive $x$-axis.
Let $(P^W_1, P^W_2, \ldots, P^W_k)$ be
the path decomposition of $S$ with respect to $W$, of order $k$.

Observe that any translate of $V$ intersects any $P^W_i$ in an interval of
it. Indeed, if
$X_1<_yX_2<_yX_3\in P^W_i$, then $X_2\in W(X_1, X_3)\cap -W(X_1, X_3)$, which
is a subset of $V(X_1, X_3)\cap -V(X_1, X_3)$. See Figure 8.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%Ezt mondja az elozo is
%
%Another crucial observation is that $W(p,r)\setminus(W(p)\cup W(r))\subset
%V(p,r)$.
%(See Figure. The lines parallel to a side of $V$ are dotted, the
%lines parallel to a side of $W$ are dashed.
%The statement is true because the big dashed parallelogram is in the dotted
%parallelogram.)
%We can use this simple observation to prove that Type Contain is \wcfx.

%\begin{claim} The following configuration is NOT possible:\\
%$a<_y b<_y c\in P^W_1, d\in P^W_2$, $\exists W_b\in Tr_k^W: b, d\in W_b$,
%$\nexists W_a\in Tr_k^W: a, d\in W_a$, $\nexists W_c\in Tr_k^W: c, d\in W_c$,
%$\exists V'\in Tr^V: a, c\in V', d\notin V'$.
%\end{claim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%

%\vskip 0.2cm

%\begin{figure}[htb]
%\begin{center}
%\scalebox{0.6}{\includegraphics{forbidden.eps}}
%\caption{$W(p,r)\setminus(W(p)\cup W(r))\subset V(p,r)$.}
%If $V'\in Tr^V$ contains $a$ and $c$, then it contains $d$ as well.}
%\end{center}
%\end{figure}

%\vskip 0.2cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{vw.eps}}
\caption{$W(X_1, X_3)\cap -W(X_1, X_3)\subset V(X_1, X_3)\cap -V(X_1, X_3)$.}
\end{center}
\end{figure}
%


We show that we can color the points of $S$ with red and blue such that
any translate of $W$ which contains at least 4 points, and any translate of $V$
which contains at least 14 points, contains points of both colors.
Consider $(P^W_1, P^W_2, P^W_3, P^W_4)$,
the path decomposition of $S$ with respect to $W$, of order $4$.
We color $P^W_1$ and $P^W_2$ such that every $W'\in Tr^W_4(S)$
contains a blue point of them, and every $V'\in Tr^V_7(P^W_1\cup P^W_2)$
contains points of both colors.
Similarly, we color $P^W_3$ and $P^W_4$ such that every $W'\in Tr^W_4(S)$
contains a red point of them, and every $V'\in Tr^V_7(P^W_3\cup P^W_4)$
contains points of both colors.
Finally, we color the rest of the points
$R=S\setminus(P^W_1\cup P^W_2\cup P^W_3\cup P^W_4)$
such that every $V'\in Tr^V_2(R)$ contains points of both colors.

Recall that for any $W'\in Tr^W_4(S)$,
$|W'\cap P^W_1|=|W'\cap P^W_2|=|W'\cap P^W_3|=|W'\cap P^W_4|=1$.
For any $X\in P^W_1$,  $Y\in P^W_2$, if there is a $W'\in Tr^W_4(S)$ with
$W'\cap P^W_1=\{X\}$ and
$W'\cap P^W_2=\{Y\}$, then
we say that $X$ and $Y$ are {\em friends}.
If $X$ (resp. $Y$) has only one friend $Y$ (resp. $X$), 
then we call it a {\em fan} (of $Y$, resp. of $X$).
If $X$ or $Y$ has at least one fan, then we say that it is a {\em star}.
Those points that are neither fans, nor stars are called {\em regular}.

For an example, see Firgure 2. On the left figure, $Y_1$ is a star, its fans are $X_2$ and $X_3$, the other points are regular. On the right, $Y_2$ is a star, its fan is $X_2$, the other points are regular.

%end of the segment is a fan of the right end, which is therefore a star.

Suppose first that all points of $P^W_1$ and $P^W_2$ are regular.
Color every third point of $P^W_1$,
red and
the others blue. In $P^W_2$, color the friends of the red points blue,
and color the rest of the points of $P^W_2$ (every third) red.
For any $W'\in Tr^W_4$, $W'\cap P^W_1$ and
$W'\cap P^W_2$ are friends, therefore, at least one of them is blue.
On the other hand,
any $V'\in Tr_7^V(P^W_1\cup P^W_2)$ contains three consecutive
points of $P^W_1$ or $P^W_2$, and they have both colors.

Suppose now that not all the points of  $P^W_1$ and $P^W_2$ are regular.
Color all stars blue.
The first and last friend of a star, in the $y$-ordering,
is either a star or a regular vertex,
the others are fans.
Color the friends of each star alternatingly, according to the
$y$-ordering, starting with blue, except the last two friends; color the last
one
blue, the previous one red.
The so far uncolored regular points of
$P^W_1$ and $P^W_2$ form pairs of intervals.
We color each such pair of interval the same way as we did in the all-regular
case,
coloring the first point of each pair of intervals red. See Figure 9.

Clearly,
if $W'\in Tr^W_4$ then it contains at least one blue point of $P^W_1\cup P^W_2$.
If $V'\in Tr_7^V(P^W_1\cup P^W_2)$, then it contains four consecutive
points of $P^W_1$ or $P^W_2$, say, $X_1, X_2, X_3, X_4$, in $P^W_1$.
If $X<_y Y<_y Z\in P^W_1\cap V'$ and $Y$ is a
star,
then $V'$ must contain all fans of $Y$ as well.
Indeed, the fans of $Y$ are in $W(X,Z)\setminus(W(X)\cup W(Z))$,
and by our earlier observations, this is in
$V(X,Z)\subset V'$.
So, if either $X_2$ or $X_3$ is a star, then
$V'$ contains
a red point, since every star has a red fan.
Since the star itself is blue, we are done in this case.
If $X_1, X_2, X_3, X_4$ contains three consecutive regular
vertices then we are done again, by the coloring rule for the regular
intervals.
So we are left with the case when $X_1$ and $X_4$ are stars, $X_2$ and $X_3$
are regular.
But in this case $V'$ also contains the common friend $Y$ of $X_2$ and $X_3$ in
$P^W_2$, which is also a regular vertex.
By the coloring rule for the regular
intervals, one of $Y$, $X_2$ and $X_3$ is red, the other two are blue, so we
are done.


\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{example.eps}}
\caption{Two examples of coloring of $P^W_1\cup P^W_2$. Friends are connected
 by edges.}
\end{center}
\end{figure}




%\vskip 0.2cm

%\begin{figure}[htb]
%\begin{center}
%\scalebox{0.66}{\includegraphics{pathcoloring.eps}}
%\hspace{0.1cm}
%\scalebox{0.66}{\includegraphics{pathcoloring2.eps}}
%\caption{Two examples of coloring}
%\end{center}
%\end{figure}

\vskip 0.2cm

For $P^W_3\cup P^W_4$ we use the same coloring rule as for
$P^W_1\cup P^W_2$ but we switch the roles of the colors.
So any $W'\in Tr_4^W$ contains at least one red point of
$P^W_3\cup P^W_4$ and any $V'\in Tr_7^V(P^W_3\cup P^W_4)$ contains both
colors.

Finally, we have to color the rest of the points
$R=S\setminus(P^W_1\cup P^W_2\cup P^W_3\cup P^W_4)$
such that every $V'\in Tr^V_2(R)$ contains points of both colors.
This can be achieved by the first proof of Lemma 1.

Now
any $W'\in Tr_4^W$ contains at least one blue and at least one red point.
If $V'\in Tr_{14}^V$, then either it contains at least two points of $R=P\setminus
(P^W_1\cup P^W_2\cup P^W_3\cup P^W_4)$,
or at least seven points of $P^W_1\cup P^W_2$, or at least seven points of
$P^W_3\cup P^W_4$, and in all cases it contains points of both colors.
This completes the proof of Lemma 2. \hfill $\Box$

\medskip

%{\bf All Types}

%The next technical result allows us to simplify all following proofs.



\noindent {\bf Definition 2.}
Suppose that ${\cal W}=\{ V, W \}$ is a pair of wedges.
$\cal W$ is said to be {\em asymmetric non-conflicting} 
or simply ANC, if there is a
constant $k$ with the
following property.
Any finite set of points $S$ can be colored with red and blue such that
any translate of $V$
that contains at least $k$ points of
$S$, contains a red point, and
any translate of $W$
that contains at least $k$ points of
$S$, contains a blue point.

\medskip

The next technical result allows us to simplify all following proofs.

\medskip

\noindent {\bf Lemma 3.} {\em If a pair of wedges is not of type Special,
and ANC, then it is also NC.}

\noindent {\bf Proof of Lemma 3.}
%Obviously, property ANC is weaker, so we only have to prove the ``only
%if'' part.
%In \cite{P08} is has been proved that if $\{V, W\}$ is a Special pair,
%then $\{V, W\}$ is {\em not} ANC. So we assume in the sequel that
%$\{V, W\}$ is not Special.
%
We can assume without loss of generality that
$V$ contains the positive $x$-axis, and $W$ contains either the positive or
the negative $x$-axis.
%
Suppose that $\{V, W\}$ is ANC, let $k>0$ arbitrary, and let $S$ be a set
of points.
First we color $Bd^V(S)$.
%We know that a translate of $V$ intersects $Bd^V(S)$ in an interval.
Let $U$ be a wedge that also contains the
positive $x$-axis, but has a very small angle.
Then translates of $V$ and translates of
$U$ both intersect  $Bd^V(S)$ in its intervals.
Clearly, the pair $\{U, W\}$ is of type Contain, therefore, by Lemma 2,
we can color  $Bd^V(S)$ such that any translate of $W$,
$W'\in Tr_4^W(Bd^V(S))$ and any translate of $U$,
$U'\in Tr_{14}^U(Bd^V(S))$ contains both colors.
But then any translate of $V$,
$V'\in Tr_{14}^V(Bd^V(S))$ contains both colors as well.

Now we have to color $S\setminus Bd^V(S)$.
We divide it into three parts as follows.
%$A_B=\cup_{q\in Bd^V(P) blue} Sh^V(q)$
%$A_R=\{p\in P\setminus Bd^V(P): \exists q\in Bd^V(P) \textit{ red}: p\in Sh^V(q)\}$,\\
$$S_{\mbox{b}}=\{ X\in S\setminus Bd^V(S)\ |\  \forall Y\in V(X)\cap
Bd^V(S), Y \ {\mbox {is blue}} \},$$
$$S_{\mbox{r}}=\{ X\in S\setminus Bd^V(S)\ |\  \forall Y\in V(X)\cap
Bd^V(S), Y \ {\mbox {is red}} \},$$
$$S_0=S\setminus (Bd^V(S)\cup S_{\mbox{b}}\cup S_{\mbox{r}}).$$

Any translate $V'\in Tr^V$
that intersects $S_{\mbox{b}}$ in at least one point,
must contain at least one blue point, from $Bd^V(S)$,
so we only have to make sure that it contains a red point too.
Similarly, any
$V'\in Tr^V$ that intersects $S_{\mbox{r}}$ in at least one point,
must contain a red point,
and any $V'\in Tr^V$ that intersects $S_0$ must contain points of both colors.

Thus, we can simply color $S_0$ such that any $W'\in Tr_2^W(S_0)$ contains
both colors, which can be done by Lemma 1.

With  $S_{\mbox{b}}$, and with $S_{\mbox{r}}$, respectively, we proceed
exactly the same way as we did with $S$ itself, but now we change the roles of
$V$ and $W$.
We get the (still uncolored)
subsets $S_{\mbox{b,b}}$, $S_{\mbox{b,r}}$, $S_{{\mbox{b}},0}$,
$S_{\mbox{r,b}}$, $S_{\mbox{r,r}}$, $S_{{\mbox{r}},0}$
with the following properties.

\begin{itemize}
\item Any translate $V'\in Tr^V$ or $W'\in Tr^W$,
that intersects  $S_{\mbox{b,b}}$
(resp. $S_{\mbox{r,r}}$)
in at least one point,
must contain at least one blue (resp. red) point.

\item Any translate $V'\in Tr^V$
that intersects  $S_{\mbox{b,r}}$
(resp. $S_{\mbox{r,b}}$)
contains a blue (resp. red) point,
and any translate $W'\in Tr^W$
that intersects  $S_{\mbox{b,r}}$
(resp. $S_{\mbox{r,b}}$)
contains a red (resp. blue) point.

\item Any translate $V'\in Tr^V$
that intersects  $S_{{\mbox{b}},0}$
(resp. $S_{{\mbox{r}},0}$)
contains a blue (resp. red) point,
and any translate $W'\in Tr^W$
that intersects  $S_{{\mbox{b}},0}$
(resp. $S_{{\mbox{r}},0}$)
contains points of both colors.

\end{itemize}

Color all points of
$S_{\mbox{b,b}}$ and $S_{{\mbox{b}},0}$ red, color
all points of $S_{\mbox{r,r}}$ and $S_{{\mbox{r}},0}$ blue.
Finally, color $S_{\mbox{b,r}}$ using the ANC property of the pair
$(V, W)$, and similarly, color $S_{\mbox{r,b}}$ also using the ANC
property, but the roles of red and blue switched.
Now it is easy to check that in this coloring any translate of $V$ or $W$ that
contains sufficiently many points of $S$, contains a point of both colors. \hfill $\Box$

%To see that this coloring is indeed correct, let us prove that any $W'\in
%Tr^W_{k}(P)$ contains both colors.
%If it intersects $Bd^V(P)$ in at least $4$ points, then we are done.
%Otherwise $W'\in Tr^W_{k-3}(P\setminus Bd^V(P))$. If it intersects $A_0$ in
%at least $2$ points,
%we are done again. Otherwise it contains at least $\frac{k}{2}-2$ points form
%$A_R$ or $A_B$.
%Since the two cases are symmetric, wlog. $W'\in Tr^W_{\frac{k}{2}-2}(A_R)$.
%Now if it intersects $Bd^W(A_R)$ in at least $14$ points, we are done, it
%must contain both colors.
%Otherwise it contains at least one at at most $13$ red or $13$ blue points
%but not both (or we are done).
%In the first case it contains at least $\frac{k}{2}-15$ points from $A_{RR}$,
%but all points are blue there, so we are done if $k\ge 31$.
%In the second case $W'\in Tr^W_{\frac{k}{2}-15}(A_{RB})$, so we need that $V$ and $W$ are
%\dwcf for $\frac{k}{2}-15$, we can pick $k$ to be sufficiently large and we
%are done.

\medskip

\noindent {\bf Remark.} In \cite{P10} it has been proved that if $\{V, W\}$
is a Special pair,
then $\{V, W\}$ is {\em not} ANC. So, the following statement
holds as well.

\smallskip

\noindent {\bf Lemma 3'.} {\em If a pair of wedges is
ANC, then it is also NC.}

\bigskip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent {\bf Lemma 4.} {\em Let ${\cal W}=\{ V, W\}$ be
a set of two wedges, of type 1 (Big).
Then $\cal W$ is NC.}

\smallskip

\noindent {\bf Proof of Lemma 4.} By Lemma 3, it is enough to show that $\{ V, W\}$ is ANC. Let $W$ be the
wedge whose angle is at least $\pi$. Then $W$ is the union of two halfplanes,
say, $H_1$ and $H_2$. Translate both halfplanes such that they contain exactly
one point of $S$, denote them by
$X_1$ and $X_2$, respectively. Note that $X_1$ may coincide with $X_2$.
Color $X_1$ and $X_2$ red, and all the other points blue.
Then any translate of $W$ that contains at least one point, contains a red
point, and any translate of $V$ that contains at least three points, contains
a blue point.
\hfill $\Box$

\medskip

\noindent {\bf Lemma 5.} {\em Let ${\cal W}=\{ V, W\}$ be
a set of two wedges, of type 2 (Halfplane).
Then $\cal W$ is NC.}

\smallskip

\noindent {\bf Proof of Lemma 5.}
Again, it is enough to show that they are ANC. Since $\{ V, W\}$ is
of type 2 (Halfplane),
$Bd^V(S)$ and $Bd^W(S)$ have at most one point in
common.
If $Bd^V(S)$ and $Bd^W(S)$ are disjoint, then color  $Bd^V(S)$ blue,
$Bd^W(S)$ red, and the other points arbitrarily.
Then any nonempty translate of $V$ (resp. $W$) contains a blue (resp. red) point.

Otherwise, let $X$ be their common point.
Let $P=Bd^V(S)\cup Bd^W(S)\setminus X$, and consider its $V$-boundary,
$Bd^V(P)$, and $W$-boundary,
$Bd^W(P)$.
Clearly, each point in $P=Bd^V(S)\setminus X$ belongs to $Bd^V(P)$,
and each point in $P=Bd^W(S)\setminus X$ belongs to $Bd^W(P)$.

If $Bd^V(P)$ and
$Bd^W(P)$ are disjoint, then color  $Bd^V(S)$ blue,
$Bd^W(P)$ and the other points red.
Then any nonempty translate of $V$ contains a blue point.
Suppose that we have a translate of $W$ with two points,
both blue. Then it should contain $X$, and a point
of  $Bd^V(P)$. But this contradicts our assumption that
$Bd^V(P)$ and
$Bd^W(P)$ are disjoint.
So, any
translate of $W$ which contains at least two points of
$S$,
contains a red point.

If $Bd^V(P)$ and
$Bd^W(P)$ are not disjoint,
then they have one point in common, let
$Y$ be their common point.
If $Y$ belongs to $Bd^W(P)$, then color
$Bd^V(S)$ blue,
$Bd^W(P)$ and the other points red.
Then, by the same argument as before,
any nonempty translate of $V$ contains a blue point, and
any
translate of $W$ which contains at least two points of
$S$,
contains a red point.
Finally, if $Y$ belongs to $Bd^V(P)$, then we proceed
analogously, but the roles of $V$ and $W$, and
the colors, are switched. \hfill $\Box$

\medskip

\noindent {\bf Lemma 6.} {\em Let ${\cal W}=\{ V, W\}$ be
a set of two wedges, of type 4 (Hard).
Then $\cal W$ is NC.}

\smallskip

\noindent {\bf Proof of Lemma 6.}
As usual, we only prove that $\{ V, W\}$ is ANC.
Assume that
$W$ contains the positive $x$-axis.
Just like in the definition of type 4 (Hard),
extend the boundary halflines of $W$ to lines,
they divide the plane
into four parts, Upper, Lower, Left, and Right, which is $W$ itself.
We can assume without loss of generality that
$V$ contains the negative $x$-axis, one side of $V$ is in Upper, and one side
is in Left.

Observe that if a translate of $V$ and a translate of $W$ intersect each
other, then
one of them contains the other one's apex.

\smallskip

{\bf Claim 1.} For any point set $P$ and $X\in P$,
either $Bd^V(P\setminus X)\setminus Bd^V(P)=\emptyset$ or $Bd^W(P\setminus X)\setminus Bd^W(P)=\emptyset$.

\smallskip

{\bf Proof of Claim 1.} Suppose on the contrary that
$Y\in Bd^V(P\setminus X)\setminus Bd^V(P)$ and $Z\in Bd^W(P\setminus X)\setminus Bd^W(P)$.
Then $X\in V(Y)$ and $X\in W(Z)$, so $V(Y)$ and $W(Z)$ intersect each other,
therefore, one of them contains the other one's apex, say,
$Z\in V(Y)$. But this is a contradiction, since $Y$ is a boundary point of
$P\setminus X$.

\smallskip

Return to the proof of Lemma 6.
Color
$Bd^V(S)\setminus Bd^W(S)$ red, and
$Bd^W(S)\setminus Bd^V(S)$ blue, the interior points arbitrarily.
Now consider the points of $Bd^V(S)\cap Bd^W(S)$.
For any $X\in Bd^V(S)\cap Bd^W(S)$,
if
$Bd^V(S\setminus X)\setminus Bd^V(S)\ne\emptyset$, then color it red,
if $Bd^W(S\setminus X)\setminus Bd^W(S)\ne\emptyset$, then color it blue.
For each of the remaining points $Y$ we have
$Bd^V(S\setminus Y)\setminus Bd^V(S)=
 Bd^W(S\setminus Y)\setminus Bd^W(S)=\emptyset$.
Color each of these points such that they have
the {\em opposite} color than the the previous point
of $Bd^V(S)\cap Bd^W(S)$,
in the $y$-ordering.

To prove that this coloring is
good, let
$V'\in Tr_2^V$, $V'\cap S = \{ X, Y\}$.
If it intersects $Bd^V(S)\setminus Bd^W(S)$, we are done.
So assume that $V'\cap Bd^V(S)\subset Bd^V(S)\cap Bd^W(S)$.
Let $X\in V'\cap Bd^V(S)$. If $X$ is red, then by the coloring rule,
$Bd^V(S\setminus X)\setminus Bd^V(S)=\emptyset$. But then $Y$ is also a
$V$-boundary point, so
we have $Y\in  Bd^V(S)\cap Bd^W(S)$. Again we can assume that $Y$ is
red, so
$Bd^V(S\setminus Y)\setminus Bd^V(S)=\emptyset$.
Suppose that $X<_yY$. Since $V'\cap S = \{ X, Y\}$, $X$ and $Y$ are
consecutive points of $Bd^V(S)\cap Bd^W(S)$.
Now it is not hard to see that
$Bd^W(S\setminus Y)\setminus Bd^W(S)=\emptyset$. Therefore, by the coloring
rule, $X$ and $Y$ have different colors.
For translates of $W$ the argument is analogous, with the colors switched.
\hfill $\Box$

\medskip

Now we turn to the case when we have more than two wedges.

\medskip

\noindent {\bf Lemma 7.} {\em For any $s, t>0$ integers, there is a number $f(s, t)$ with the
following property.

Let ${\cal W}=\{ W_1, W_2, \ldots , W_t \}$ be a set of $t$ wedges, such that
any pair $\{W_i, W_j \}$ is NC, and let $S$ be a set of points.
Then $S$ can be decomposed into $t$ parts, $S_1, S_2, \ldots , S_t$, such that
for $i=1, 2, \ldots , t$, for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S|\ge f(s, t)$ then
$|W'_i\cap S_i|\ge s$.}

% Dual, alt helyzet, loc finite (triangle-bol) f(1, 2)=?

\medskip

\noindent {\bf Proof of Lemma 7.}
The existence of $f(1,2)$ is equivalent to the property that
the corresponding two wedges are ANC.
Now we show that $f(s, 2)$ exists for every $s$.
Let $V$ and $W$ be two wedges that form a NC pair.
Let $P^V_1, P^V_2, \ldots , P^V_{s^2f(1,2)}$ be the path decomposition
of $S$ of order $s^2f(1,2)$, with respect to $V$.
For $i=1, 2, \ldots , s$, let
$$H_i=\cup_{j=(i-1)sf(1,2)+1}^{isf(1,2)} P_j^V.$$
For each $H_i$, take the $W$-path decomposition, $P_1^W(H_i),\ldots,
P_{sf(1,2)}^W(H_i)$, and for $j=1, 2, \ldots , s$, let
$$H_i^j=\cup_{k=(j-1)f(1,2)+1}^{jf(1,2)} P_k^W(H_i).$$
For every
$i, j=1, 2, \ldots , s$,
color $H_i^j$, such that any translate of $V$ (resp. $W$) that intersects it
in at least $f(1,2)$ points,
contains at least one red (resp. blue) point of it. This is possible, since
the
pair $\{ V, W\}$ is ANC.

Consider a translate $V'$ of $V$ that
contains at least $s^2f(1,2)$ points of $S$.
For every $i$, $V'$ intersects $H_i$ in
$sf(1,2)$ points, so there is a $j$ such that
it intersects $H_i^j$ in at least $f(1,2)$
points. Therefore, $V'$ contains at least one red point
of $H_i^j$, so at least $s$ red points of $S$.

Consider now a translate $W'$ of $W$ that
contains at least $s^2f(1,2)$ points of $S$.
There is an $i$ such that
$W'$ intersects $H_i$ in at least $sf(1,2)$
points. Therefore, it intersects
each of $P_1^W(H_i),\ldots,
P_{sf(1,2)}^W(H_i)$, in at least one point, so
for $j=1, 2, \ldots, s$, $W'$ intersects
$H_i^j$ in at least $f(1,2)$ points. Consequently,
it contains at least one blue point of each
$H_i^j$, so at least $s$ blue points of $S$.

\smallskip

Now let $s, t>2$ fixed and suppose that $f(s',t-1)$ exists for every $s'$.
Let $\{W_1, W_2, \ldots , W_t\}$ be our set of wedges, such that any pair
of them is NC. Let $s'=f(s, 2)$.
Partition our point set $S$ into
$S'_1, S'_2, \ldots, S'_{t-1}$ such that
for $i=1, 2, \ldots , t-1$, for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S|\ge f(s', t-1)$ then
$|W'_i\cap S'_i|\ge s'=f(s, 2)$.
For each $i=1, 2, \ldots , t-1$, partition
$S'_i$ into two parts, $S''_i$ and $S^t_i$,
such that for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S'_i|\ge f(s, 2)$ then
$|W'_i\cap S''_i|\ge s$, and
for any translate $W'_t$ of $W_t$,
if $|W'_t\cap S'_i|\ge f(s, 2)$ then
$|W'_t\cap S^t_i|\ge s$.
Finally,
for $i=1, 2, \ldots , t-1$, let $S_i=S''_i$ and
let $S_t=\cup_{j=1}^{t-1}S^t_j$.
For $i=1, 2, \ldots , t-1$,
any translate $W'_i$ of $W_i$, if
$|W'_i\cap S|\ge f(s', t-1)$ then
$|W'_i\cap S'_i|\ge s'=f(s, 2)$, so
$|W'_i\cap S_i|\ge s$,

And for any translate $W'_t$ of $W_t$, if
$|W'_i\cap S|\ge f(s', t-1)$,
then for some $i=1, 2, \ldots t-1$,
$|W'_t\cap S'_i|\ge \frac{f(s', t-1)}{t-1}\ge f(s,2)$, therefore,
$|W'_t\cap S^t_i|\ge s$, so
$|W'_t\cap S_t|\ge s$.
This concludes the proof of Lemma 7. \hfill $\Box$

\smallskip

\noindent {\bf Remark.} The proofs of Lemmas 2, 4, 5, and 6 imply that
$f(1, 2)\le 8$. Combining it with the proof of Lemma 7 we get the bound
$f(s,t)\le (8s)^{2^{t-1}}$.


\medskip

\noindent {\bf Lemma 8.} {\em A set of wedges ${\cal W}=\{ W_1, W_2, \ldots ,
W_t \}$ is NC if and only if any pair $\{W_i, W_j \}$ is NC.}

\smallskip

\noindent {\bf Proof of Lemma 8.}
Clearly, if some pair $\{W_i, W_j \}$ is {\em not} NC, then the whole set
$\cal W$ is not NC either.
Suppose that every pair $\{W_i, W_j \}$ is NC.
Decompose $S$ into $t$ parts $S_1, S_2, \ldots , S_t$
with the property that
for $i=1, 2, \ldots , t$, for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S|\ge f(3, t)$ then
$|W'_i\cap S_i|\ge 3$.
Then, by Lemma 1, each $S_i$ can be colored with red and blue such
that if
$|W'_i\cap S_i|\ge 3$
then $W'_i$ contains points of both colors.
So this coloring of $S$ has the property that
for $i=1, 2, \ldots , t$, for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S|\ge f(3, t)$ then it contains points of both colors. \hfill $\Box$

% f(1,2)=?

\subsection{Proof of Theorem 1.}

Suppose that $P$ is an open convex polygon of $n$ vertices and
${\cal P}=\{\ P_i\ |\ i\in I\ \}$ is a collection of translates of
$P$ which forms an
$M$-fold covering of the plane.
We will set the value of $M$ later.
Let $m$ be the minimum distance
between any vertex and non-adjacent side of $P$.
Take a square grid $\cal G$ of basic distance $m/2$.
Obviously, any translate of $P$ intersects at most
$K=4\pi(diam(P)+m)^2/m^2$ basic squares.
For each (closed) basic square $B$, using its compactness,
we can find a {\em finite} subcollection of the translates such that
they still form an $M$-fold covering of $B$.
Take the union of all these subcollections.
We have a {\em locally finite} $M$-fold covering of the plane.
That is, every compact set is intersected by finitely many of the translates.
It is sufficient to decompose this covering.
For simplicity, use the same notation
${\cal P}=\{\ P_i\ |\ i\in I\ \}$ for this subcollection.

We formulate
and solve the problem in its dual
form.
Let $O_i$ be the center of gravity of $P_i$.
Since ${\cal P}$ is an $M$-fold covering of the plane,
every translate of $\bar{P}$, the reflection of $P$ through the
origin, contains at least $M$ points of the locally finite set
${\cal O}=\{\ O_i\ |\ i\in I\ \}$.

The collection ${\cal P}=\{\ P_i\ |\ i\in I\ \}$ can be decomposed into two
coverings
if and only if the set ${\cal O}=\{\ O_i\ |\ i\in I\ \}$ can be colored with
two colors, such that every translate of $\bar{P}$ contains a point of both
colors.

Let ${\cal W}=\{ W_1, W_2, \ldots , W_n \}$ be the set of wedges
that correspond to the vertices of $\bar{P}$.
By the convexity of $\bar{P}$,
no pair $\{W_i, W_j \}$ is of type 5 (Special), therefore,
by the previous Lemmas,
each pair is NC. Consequently, by Lemma 8, ${\cal W}$ is
NC as well. So there is a $k$ with the following property.

\smallskip

\noindent {\bf *}  Any set of points $S$ can be colored with two colors such that
any translate of $W_1, W_2, \ldots , W_n$
that contains at least $k$ points of $S$, contains points of both colors.

\smallskip

Choose $M$ such that $M\ge kK$, and color the points of
$\cal O$ in each basic square separately, with property {\bf *}.

Since any translate $P'$ of $\bar{P}$ intersects at most
%$40A(P)/m^2$
$K$ basic squares of the grid $\cal G$, $P'$ contains at least $M/K\ge k$ points of
${\cal O}$ in the same basic square $B'$.
By the choice of the grid $\cal G$,
$B'$ contains at most one vertex of $P'$, hence
$B'\cap P'=B'\cap W$, where $W$ is a translate
of some $W_i\in {\cal W}$. So, by property {\bf *},
$P'$ contains points of ${\cal O}\cap B'$ of both colors.
This concludes the proof of Theorem 1. \hfill $\Box$

%\noindent {\bf Remark.} 
%\begin{remark} If we want to decompose a covering by the translates of a
%$t$-gon into $s$-parts, then we need that $M\ge f(s,t)K$. Therefore in this
%case a $K(8s)^{2^{t-1}}$-fold covering 
%suffices.
%\end{remark}


\subsection{Concluding Remarks}
Throughout this paper we made no attempt to optimize the constants.
However, it may be 
an
interesting problem to determine (asymptotically) 
the smallest $k$ in the proof of
Theorem 1. 

Another interesting question is to decide whether
this constant depends only on the number of vertices of the polygon or on the
shape as well. In particular, we cannot verify the following.

\medskip

\noindent {\bf Conjecture.} {\em There is a constant $k$ such that any
$k$-fold covering of the plane with translates of a
convex quadrilateral
can be decomposed into two coverings.}

\medskip

One can also investigate whether a given covering can be decomposed into
$s$ coverings, for some fixed $s$. 
For any planar set $P$ and $s\ge 1$, if it exists, 
let $k=k(s, P)$ be the smallest 
number such that any $k$-fold covering of the plane with translates of
$P$ can be decomposed into $s$ coverings. 
By Theorem 1, $k(2, P)$ exists for any open convex polygon $P$.
With a slight modification 
of its proof, we get the following more general result.

\medskip

\noindent {\bf Theorem 1'.} {\em For any open convex polygon $P$, and any 
$s$, there exists a (smallest) number $k=k(s, P)$ such that 
any $k$-fold covering of the plane with translates of
$P$ can be decomposed into $s$ coverings. }

\medskip

Our proof gives $k(s, P)<K_P(8s)^{2^{n-1}}$, where $K_P$ is the constant $K$ from the
proof of Theorem 1 and $n$ is the number of vertices of $P$. 
For {\em centrally symmetric} open convex polygons 
Pach and T\'oth \cite{PT07} established 
a much better upper bound, 
which is quadratic in 
$s$.
Recently, 
Aloupis et al. \cite{A08} improved it to linear. 
They showed that, for any centrally symmetric open convex polygon
$P$, there is an $\alpha_P$ such that
$k(s, P)<\alpha_Ps$.
The best known lower bound on $k(s, P)$ is $(s, P)\ge\lfloor 4s/3\rfloor-1$
\cite{PT07}.
 
\medskip

Our proofs use the assumption that the covering is locally finite, and 
for open polygons we 
could find a locally finite subcollection which is still a $k$-fold covering.
Still, we strongly believe that Theorem 1 holds for closed convex polygons
as well.

\medskip

\noindent {\bf Acknowledgement.} We are very grateful to the anonymous
referee
for his remarks.





==> convexkulonszam.tex <==

This section is based on our paper with G\'eza T\'oth, Convex polygons are cover-decomposable.

Our main result is Theorem A. (iii), restated as

\medskip

\noindent {\bf Theorem 1.} {\em Every open convex polygon
is cover-decomposable.}

\medskip



In Section 2 we prove some results about coloring point sets with respect to
translates of wedges. In Section 3 we formulate the problem precisely
in the dual version, and apply the results of Section 2 to prove Theorem 1.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Preparation}

Now let $W$ be a wedge, and $X$ be a point in the plane. A translate of $W$
such that its apex is at $X$, is denoted by $W(X)$.
More generally, for points $X_1, X_2, \ldots X_k$,
$W(X_1, X_2, \ldots X_k)$ denotes the {\em minimal} translate of $W$
(for containment) whose
closure
contains $X_1, X_2, \ldots X_k$.
The set of all translates
of $W$ is denoted by $Tr^W$ and the set of those translates that contain exactly $k$ points from a point set $S$ is denoted by $Tr^W_k(S)$.
Let $-W$ denote the reflection of $W$ about the origin.

We can assume without loss of generality that the positive $x$-axis is in $W$, and that no two points from our point set, $S$, have the same $y$-coordinate.
Both of these can be achieved by an appropriate rotation.
We say that $X<_yY$ if the $y$-coordinate of $X$ is smaller than the
$y$-coordinate of $Y$. This ordering is called the $y$-ordering.
A subset $I$ of $S$ is an {\em interval} of $S$
if $\forall X<_y Y<_y Z\in S: X,Z\in I \rightarrow Y\in I.$

The {\em boundary} of $S$ with respect to $W$,
$Bd^W(S)=\{X\in P:W(X)\cap S=\emptyset\}.$
Note that a translate of $W$ always intersects the boundary in an interval.
For each $X\in Bd^W(S)$ the {\em shadow} of $X$ is
$Sh^W(X)=\{Y\in S: W(Y)\cap Bd^W(S)=X\}.$
Observe that $\forall X,Y\in Bd^W(S): Sh^W(X)\cap Sh^W(Y)=\emptyset.$

Now we give another proof using these notions for Lemma \ref{1wedge}.
In fact, we show that if the angle of $W$ is less than $\pi$, then the points of $S$ can be colored with two colors such that any wedge that has at least two points contains both colors (so the NC property holds with $k=2$).

\medskip

\noindent {\bf Proof.} Color the points of the boundary alternating, according to the order $<_y$.
For every boundary point $X$,
color every point in the shadow of $X$ to the other color than $X$.
Color the rest of the points arbitrarily.
Any translate of $W$ that contains at least two points,
contains one or two boundary points.
If it contains one boundary point, then the other point is in its shadow,
so they have different colors.
If it contains two boundary points, then they are consecutive points according
to the $y$-order, so they have different colors again. \hfill $\Box$.

\smallskip

Now we can turn to the case when we have
translates of two or more wedges at the same time.
Remember that any pair of wedges belong to a Type determined by their relative
position. The different types are classified in Section \ref{sec:class} and are depicted in Figures \ref{fig:type2}, \ref{fig:type3}, \ref{fig:type4}, \ref{fig:type5}.
It is shown in \cite{P10} that if ${\cal W}=\{ V, W\}$ is a set of two wedges
of Type 5 (Special), then $\cal W$ is {\em not} NC. In a series of lemmas we show that all
other pairs are NC, thus proving Lemma \ref{2wedge}.

\medskip

\noindent {\bf Lemma 2.} {\em Let ${\cal W}=\{ V, W\}$ be
a set of two wedges, of Type 3 (Contain).
Then $\cal W$ is NC.}

\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{t3.eps}}
\caption{Type 3 (Contain)}
\end{center}
\end{figure}

\medskip


\noindent {\bf Proof of Lemma 2.}
We can assume that $W\supset V$ or  $W\supset -V$
and $W$ contains the positive $x$-axis.
Let $(P^W_1, P^W_2, \ldots, P^W_k)$ be
the path decomposition of $S$ with respect to $W$, of order $k$.

Observe that any translate of $V$ intersects any $P^W_i$ in an interval of
it. Indeed, if
$X_1<_yX_2<_yX_3\in P^W_i$, then $X_2\in W(X_1, X_3)\cap -W(X_1, X_3)$, which
is a subset of $V(X_1, X_3)\cap -V(X_1, X_3)$. See Figure \ref{fig:vw}.


\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{vw.eps}}
\caption{$W(X_1, X_3)\cap -W(X_1, X_3)\subset V(X_1, X_3)\cap -V(X_1, X_3)$.}
\label{fig:vw}
\end{center}
\end{figure}
%


We show that we can color the points of $S$ with red and blue such that
any translate of $W$ which contains at least 4 points, and any translate of $V$
which contains at least 14 points, contains points of both colors.
Consider $(P^W_1, P^W_2, P^W_3, P^W_4)$,
the path decomposition of $S$ with respect to $W$, of order $4$.
We color $P^W_1$ and $P^W_2$ such that every $W'\in Tr^W_4(S)$
contains a blue point of them, and every $V'\in Tr^V_7(P^W_1\cup P^W_2)$
contains points of both colors.
Similarly, we color $P^W_3$ and $P^W_4$ such that every $W'\in Tr^W_4(S)$
contains a red point of them, and every $V'\in Tr^V_7(P^W_3\cup P^W_4)$
contains points of both colors.
Finally, we color the rest of the points
$R=S\setminus(P^W_1\cup P^W_2\cup P^W_3\cup P^W_4)$
such that every $V'\in Tr^V_2(R)$ contains points of both colors.

Recall that for any $W'\in Tr^W_4(S)$,
$|W'\cap P^W_1|=|W'\cap P^W_2|=|W'\cap P^W_3|=|W'\cap P^W_4|=1$.
For any $X\in P^W_1$,  $Y\in P^W_2$, if there is a $W'\in Tr^W_4(S)$ with
$W'\cap P^W_1=\{X\}$ and
$W'\cap P^W_2=\{Y\}$, then
we say that $X$ and $Y$ are {\em friends}.
If $X$ (resp. $Y$) has only one friend $Y$ (resp. $X$), 
then we call it a {\em fan} (of $Y$, resp. of $X$).
If $X$ or $Y$ has at least one fan, then we say that it is a {\em star}.
Those points that are neither fans, nor stars are called {\em regular}.

For an example, see Figure \ref{fig:path2}. On the left figure, $Y_1$ is a star, its fans are $X_2$ and $X_3$, the other points are regular. On the right, $Y_2$ is a star, its fan is $X_2$, the other points are regular.


Suppose first that all points of $P^W_1$ and $P^W_2$ are regular.
Color every third point of $P^W_1$,
red and
the others blue. In $P^W_2$, color the friends of the red points blue,
and color the rest of the points of $P^W_2$ (every third) red.
For any $W'\in Tr^W_4$, $W'\cap P^W_1$ and
$W'\cap P^W_2$ are friends, therefore, at least one of them is blue.
On the other hand,
any $V'\in Tr_7^V(P^W_1\cup P^W_2)$ contains three consecutive
points of $P^W_1$ or $P^W_2$, and they have both colors.

Suppose now that not all the points of  $P^W_1$ and $P^W_2$ are regular.
Color all stars blue.
The first and last friend of a star, in the $y$-ordering,
is either a star or a regular vertex,
the others are fans.
Color the friends of each star alternatingly, according to the
$y$-ordering, starting with blue, except the last two friends; color the last
one
blue, the previous one red.
The so far uncolored regular points of
$P^W_1$ and $P^W_2$ form pairs of intervals.
We color each such pair of interval the same way as we did in the all-regular
case,
coloring the first point of each pair of intervals red. See Figure \ref{fig:friends}.

Clearly,
if $W'\in Tr^W_4$ then it contains at least one blue point of $P^W_1\cup P^W_2$.
If $V'\in Tr_7^V(P^W_1\cup P^W_2)$, then it contains four consecutive
points of $P^W_1$ or $P^W_2$, say, $X_1, X_2, X_3, X_4$, in $P^W_1$.
If $X<_y Y<_y Z\in P^W_1\cap V'$ and $Y$ is a
star,
then $V'$ must contain all fans of $Y$ as well.
Indeed, the fans of $Y$ are in $W(X,Z)\setminus(W(X)\cup W(Z))$,
and by our earlier observations, this is in
$V(X,Z)\subset V'$.
So, if either $X_2$ or $X_3$ is a star, then
$V'$ contains
a red point, since every star has a red fan.
Since the star itself is blue, we are done in this case.
If $X_1, X_2, X_3, X_4$ contains three consecutive regular
vertices then we are done again, by the coloring rule for the regular
intervals.
So we are left with the case when $X_1$ and $X_4$ are stars, $X_2$ and $X_3$
are regular.
But in this case $V'$ also contains the common friend $Y$ of $X_2$ and $X_3$ in
$P^W_2$, which is also a regular vertex.
By the coloring rule for the regular
intervals, one of $Y$, $X_2$ and $X_3$ is red, the other two are blue, so we
are done.


\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{example.eps}}
\caption{Two examples of coloring of $P^W_1\cup P^W_2$. Friends are connected
 by edges.}
 \label{fig:friends}
\end{center}
\end{figure}

\vskip 0.2cm

For $P^W_3\cup P^W_4$ we use the same coloring rule as for
$P^W_1\cup P^W_2$ but we switch the roles of the colors.
So any $W'\in Tr_4^W$ contains at least one red point of
$P^W_3\cup P^W_4$ and any $V'\in Tr_7^V(P^W_3\cup P^W_4)$ contains both
colors.

Finally, we have to color the rest of the points
$R=S\setminus(P^W_1\cup P^W_2\cup P^W_3\cup P^W_4)$
such that every $V'\in Tr^V_2(R)$ contains points of both colors.
This can be achieved by the first proof of Lemma \ref{1wedge}.

Now
any $W'\in Tr_4^W$ contains at least one blue and at least one red point.
If $V'\in Tr_{14}^V$, then either it contains at least two points of $R=P\setminus
(P^W_1\cup P^W_2\cup P^W_3\cup P^W_4)$,
or at least seven points of $P^W_1\cup P^W_2$, or at least seven points of
$P^W_3\cup P^W_4$, and in all cases it contains points of both colors.
This completes the proof of Lemma 2. \hfill $\Box$

\medskip

\noindent {\bf Definition 2.}
Suppose that ${\cal W}=\{ V, W \}$ is a pair of wedges.
$\cal W$ is said to be {\em asymmetric non-conflicting} 
or simply ANC, if there is a
constant $k$ with the
following property.
Any finite set of points $S$ can be colored with red and blue such that
any translate of $V$
that contains at least $k$ points of
$S$, contains a red point, and
any translate of $W$
that contains at least $k$ points of
$S$, contains a blue point.

\medskip

The next technical result allows us to simplify all following proofs.

\medskip

\noindent {\bf Lemma 3.} {\em If a pair of wedges is not of Type 5 (Special),
and ANC, then it is also NC.}

\smallskip

\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{t5.eps}}
\caption{Type 5 (Special)}
\end{center}
\end{figure}

\noindent {\bf Proof of Lemma 3.}
We can assume without loss of generality that
$V$ contains the positive $x$-axis, and $W$ contains either the positive or
the negative $x$-axis.
%
Suppose that $\{V, W\}$ is ANC, let $k>0$ arbitrary, and let $S$ be a set
of points.
First we color $Bd^V(S)$.
Let $U$ be a wedge that also contains the
positive $x$-axis, but has a very small angle.
Then translates of $V$ and translates of
$U$ both intersect  $Bd^V(S)$ in its intervals.
Clearly, the pair $\{U, W\}$ is of type Contain, therefore, by Lemma 2,
we can color  $Bd^V(S)$ such that any translate of $W$,
$W'\in Tr_4^W(Bd^V(S))$ and any translate of $U$,
$U'\in Tr_{14}^U(Bd^V(S))$ contains both colors.
But then any translate of $V$,
$V'\in Tr_{14}^V(Bd^V(S))$ contains both colors as well.

Now we have to color $S\setminus Bd^V(S)$.
We divide it into three parts as follows.
%$A_B=\cup_{q\in Bd^V(P) blue} Sh^V(q)$
%$A_R=\{p\in P\setminus Bd^V(P): \exists q\in Bd^V(P) \textit{ red}: p\in Sh^V(q)\}$,\\
$$S_{\mbox{b}}=\{ X\in S\setminus Bd^V(S)\ |\  \forall Y\in V(X)\cap
Bd^V(S), Y \ {\mbox {is blue}} \},$$
$$S_{\mbox{r}}=\{ X\in S\setminus Bd^V(S)\ |\  \forall Y\in V(X)\cap
Bd^V(S), Y \ {\mbox {is red}} \},$$
$$S_0=S\setminus (Bd^V(S)\cup S_{\mbox{b}}\cup S_{\mbox{r}}).$$

Any translate $V'\in Tr^V$
that intersects $S_{\mbox{b}}$ in at least one point,
must contain at least one blue point, from $Bd^V(S)$,
so we only have to make sure that it contains a red point too.
Similarly, any
$V'\in Tr^V$ that intersects $S_{\mbox{r}}$ in at least one point,
must contain a red point,
and any $V'\in Tr^V$ that intersects $S_0$ must contain points of both colors.

Thus, we can simply color $S_0$ such that any $W'\in Tr_2^W(S_0)$ contains
both colors, which can be done by Lemma \ref{1wedge}.

With  $S_{\mbox{b}}$, and with $S_{\mbox{r}}$, respectively, we proceed
exactly the same way as we did with $S$ itself, but now we change the roles of
$V$ and $W$.
We get the (still uncolored)
subsets $S_{\mbox{b,b}}$, $S_{\mbox{b,r}}$, $S_{{\mbox{b}},0}$,
$S_{\mbox{r,b}}$, $S_{\mbox{r,r}}$, $S_{{\mbox{r}},0}$
with the following properties.

\begin{itemize}
\item Any translate $V'\in Tr^V$ or $W'\in Tr^W$,
that intersects  $S_{\mbox{b,b}}$
(resp. $S_{\mbox{r,r}}$)
in at least one point,
must contain at least one blue (resp. red) point.

\item Any translate $V'\in Tr^V$
that intersects  $S_{\mbox{b,r}}$
(resp. $S_{\mbox{r,b}}$)
contains a blue (resp. red) point,
and any translate $W'\in Tr^W$
that intersects  $S_{\mbox{b,r}}$
(resp. $S_{\mbox{r,b}}$)
contains a red (resp. blue) point.

\item Any translate $V'\in Tr^V$
that intersects  $S_{{\mbox{b}},0}$
(resp. $S_{{\mbox{r}},0}$)
contains a blue (resp. red) point,
and any translate $W'\in Tr^W$
that intersects  $S_{{\mbox{b}},0}$
(resp. $S_{{\mbox{r}},0}$)
contains points of both colors.

\end{itemize}

Color all points of
$S_{\mbox{b,b}}$ and $S_{{\mbox{b}},0}$ red, color
all points of $S_{\mbox{r,r}}$ and $S_{{\mbox{r}},0}$ blue.
Finally, color $S_{\mbox{b,r}}$ using the ANC property of the pair
$(V, W)$, and similarly, color $S_{\mbox{r,b}}$ also using the ANC
property, but the roles of red and blue switched.
Now it is easy to check that in this coloring any translate of $V$ or $W$ that
contains sufficiently many points of $S$, contains a point of both colors. \hfill $\Box$

\medskip

\noindent {\bf Remark.} In \cite{P10} it has been proved that if $\{V, W\}$
is a Special pair,
then $\{V, W\}$ is {\em not} ANC. So, the following statement
holds as well.

\smallskip

\noindent {\bf Lemma 3'.} {\em If a pair of wedges is
ANC, then it is also NC.}

\bigskip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent {\bf Lemma 4.} {\em Let ${\cal W}=\{ V, W\}$ be
a set of two wedges, of Type 1 (Big).
Then $\cal W$ is NC.}

\smallskip

\noindent {\bf Proof of Lemma 4.} By Lemma 3, it is enough to show that $\{ V, W\}$ is ANC. Let $W$ be the
wedge whose angle is at least $\pi$. Then $W$ is the union of two halfplanes,
say, $H_1$ and $H_2$. Translate both halfplanes such that they contain exactly
one point of $S$, denote them by
$X_1$ and $X_2$, respectively. Note that $X_1$ may coincide with $X_2$.
Color $X_1$ and $X_2$ red, and all the other points blue.
Then any translate of $W$ that contains at least one point, contains a red
point, and any translate of $V$ that contains at least three points, contains
a blue point.
\hfill $\Box$

\medskip

\noindent {\bf Lemma 5.} {\em Let ${\cal W}=\{ V, W\}$ be
a set of two wedges, of Type 2 (Halfplane).
Then $\cal W$ is NC.}

\smallskip
\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{t2.eps}}
\caption{Type 2 (Halfplane)}
\end{center}
\end{figure}

\noindent {\bf Proof of Lemma 5.}
Again, it is enough to show that they are ANC. Since $\{ V, W\}$ is
of type 2 (Halfplane),
$Bd^V(S)$ and $Bd^W(S)$ have at most one point in
common.
If $Bd^V(S)$ and $Bd^W(S)$ are disjoint, then color  $Bd^V(S)$ blue,
$Bd^W(S)$ red, and the other points arbitrarily.
Then any nonempty translate of $V$ (resp. $W$) contains a blue (resp. red) point.

Otherwise, let $X$ be their common point.
Let $P=Bd^V(S)\cup Bd^W(S)\setminus X$, and consider its $V$-boundary,
$Bd^V(P)$, and $W$-boundary,
$Bd^W(P)$.
Clearly, each point in $P=Bd^V(S)\setminus X$ belongs to $Bd^V(P)$,
and each point in $P=Bd^W(S)\setminus X$ belongs to $Bd^W(P)$.

If $Bd^V(P)$ and
$Bd^W(P)$ are disjoint, then color  $Bd^V(S)$ blue,
$Bd^W(P)$ and the other points red.
Then any nonempty translate of $V$ contains a blue point.
Suppose that we have a translate of $W$ with two points,
both blue. Then it should contain $X$, and a point
of  $Bd^V(P)$. But this contradicts our assumption that
$Bd^V(P)$ and
$Bd^W(P)$ are disjoint.
So, any
translate of $W$ which contains at least two points of
$S$,
contains a red point.

If $Bd^V(P)$ and
$Bd^W(P)$ are not disjoint,
then they have one point in common, let
$Y$ be their common point.
If $Y$ belongs to $Bd^W(P)$, then color
$Bd^V(S)$ blue,
$Bd^W(P)$ and the other points red.
Then, by the same argument as before,
any nonempty translate of $V$ contains a blue point, and
any
translate of $W$ which contains at least two points of
$S$,
contains a red point.
Finally, if $Y$ belongs to $Bd^V(P)$, then we proceed
analogously, but the roles of $V$ and $W$, and
the colors, are switched. \hfill $\Box$

\medskip

\noindent {\bf Lemma 6.} {\em Let ${\cal W}=\{ V, W\}$ be
a set of two wedges, of Type 4 (Hard).
Then $\cal W$ is NC.}

\smallskip

\begin{figure}[htb]
\begin{center}
\scalebox{0.5}{\includegraphics{t4.eps}}
\caption{Type 4 (Hard)}
\end{center}
\end{figure}

\noindent {\bf Proof of Lemma 6.}
As usual, we only prove that $\{ V, W\}$ is ANC.
Assume that
$W$ contains the positive $x$-axis.
Just like in the definition of the different types,
extend the boundary halflines of $W$ to lines,
they divide the plane
into four parts, Upper, Lower, Left, and Right, which is $W$ itself.
We can assume without loss of generality that
$V$ contains the negative $x$-axis, one side of $V$ is in Upper, and one side
is in Left.

Observe that if a translate of $V$ and a translate of $W$ intersect each
other, then
one of them contains the other one's apex.

\smallskip

{\bf Claim 1.} For any point set $P$ and $X\in P$,
either $Bd^V(P\setminus X)\setminus Bd^V(P)=\emptyset$ or $Bd^W(P\setminus X)\setminus Bd^W(P)=\emptyset$.

\smallskip

{\bf Proof of Claim 1.} Suppose on the contrary that
$Y\in Bd^V(P\setminus X)\setminus Bd^V(P)$ and $Z\in Bd^W(P\setminus X)\setminus Bd^W(P)$.
Then $X\in V(Y)$ and $X\in W(Z)$, so $V(Y)$ and $W(Z)$ intersect each other,
therefore, one of them contains the other one's apex, say,
$Z\in V(Y)$. But this is a contradiction, since $Y$ is a boundary point of
$P\setminus X$.

\smallskip

Return to the proof of Lemma 6.
Color
$Bd^V(S)\setminus Bd^W(S)$ red, and
$Bd^W(S)\setminus Bd^V(S)$ blue, the interior points arbitrarily.
Now consider the points of $Bd^V(S)\cap Bd^W(S)$.
For any $X\in Bd^V(S)\cap Bd^W(S)$,
if
$Bd^V(S\setminus X)\setminus Bd^V(S)\ne\emptyset$, then color it red,
if $Bd^W(S\setminus X)\setminus Bd^W(S)\ne\emptyset$, then color it blue.
For each of the remaining points $Y$ we have
$Bd^V(S\setminus Y)\setminus Bd^V(S)=
 Bd^W(S\setminus Y)\setminus Bd^W(S)=\emptyset$.
Color each of these points such that they have
the {\em opposite} color than the the previous point
of $Bd^V(S)\cap Bd^W(S)$,
in the $y$-ordering.

To prove that this coloring is
good, let
$V'\in Tr_2^V$, $V'\cap S = \{ X, Y\}$.
If it intersects $Bd^V(S)\setminus Bd^W(S)$, we are done.
So assume that $V'\cap Bd^V(S)\subset Bd^V(S)\cap Bd^W(S)$.
Let $X\in V'\cap Bd^V(S)$. If $X$ is red, then by the coloring rule,
$Bd^V(S\setminus X)\setminus Bd^V(S)=\emptyset$. But then $Y$ is also a
$V$-boundary point, so
we have $Y\in  Bd^V(S)\cap Bd^W(S)$. Again we can assume that $Y$ is
red, so
$Bd^V(S\setminus Y)\setminus Bd^V(S)=\emptyset$.
Suppose that $X<_yY$. Since $V'\cap S = \{ X, Y\}$, $X$ and $Y$ are
consecutive points of $Bd^V(S)\cap Bd^W(S)$.
Now it is not hard to see that
$Bd^W(S\setminus Y)\setminus Bd^W(S)=\emptyset$. Therefore, by the coloring
rule, $X$ and $Y$ have different colors.
For the translates of $W$ the argument is analogous, with the colors switched.\hfill $\Box$

\medskip

Now we turn to the case when we have more than two wedges.

\medskip

\noindent {\bf Lemma 7.} {\em For any $s, t>0$ integers, there is a number $f(s, t)$ with the
following property.

Let ${\cal W}=\{ W_1, W_2, \ldots , W_t \}$ be a set of $t$ wedges, such that
any pair $\{W_i, W_j \}$ is NC, and let $S$ be a set of points.
Then $S$ can be decomposed into $t$ parts, $S_1, S_2, \ldots , S_t$, such that
for $i=1, 2, \ldots , t$, for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S|\ge f(s, t)$ then
$|W'_i\cap S_i|\ge s$.}

\medskip

\noindent {\bf Proof of Lemma 7.}
The existence of $f(1,2)$ is equivalent to the property that
the corresponding two wedges are ANC.
Now we show that $f(s, 2)$ exists for every $s$.
Let $V$ and $W$ be two wedges that form a NC pair.
Let $P^V_1, P^V_2, \ldots , P^V_{s^2f(1,2)}$ be the path decomposition
of $S$ of order $s^2f(1,2)$, with respect to $V$.
For $i=1, 2, \ldots , s$, let
$$H_i=\cup_{j=(i-1)sf(1,2)+1}^{isf(1,2)} P_j^V.$$
For each $H_i$, take the $W$-path decomposition, $P_1^W(H_i),\ldots,
P_{sf(1,2)}^W(H_i)$, and for $j=1, 2, \ldots , s$, let
$$H_i^j=\cup_{k=(j-1)f(1,2)+1}^{jf(1,2)} P_k^W(H_i).$$
For every
$i, j=1, 2, \ldots , s$,
color $H_i^j$, such that any translate of $V$ (resp. $W$) that intersects it
in at least $f(1,2)$ points,
contains at least one red (resp. blue) point of it. This is possible, since
the
pair $\{ V, W\}$ is ANC.

Consider a translate $V'$ of $V$ that
contains at least $s^2f(1,2)$ points of $S$.
For every $i$, $V'$ intersects $H_i$ in
$sf(1,2)$ points, so there is a $j$ such that
it intersects $H_i^j$ in at least $f(1,2)$
points. Therefore, $V'$ contains at least one red point
of $H_i^j$, so at least $s$ red points of $S$.

Consider now a translate $W'$ of $W$ that
contains at least $s^2f(1,2)$ points of $S$.
There is an $i$ such that
$W'$ intersects $H_i$ in at least $sf(1,2)$
points. Therefore, it intersects
each of $P_1^W(H_i),\ldots,
P_{sf(1,2)}^W(H_i)$, in at least one point, so
for $j=1, 2, \ldots, s$, $W'$ intersects
$H_i^j$ in at least $f(1,2)$ points. Consequently,
it contains at least one blue point of each
$H_i^j$, so at least $s$ blue points of $S$.

\smallskip

Now let $s, t>2$ fixed and suppose that $f(s',t-1)$ exists for every $s'$.
Let $\{W_1, W_2, \ldots , W_t\}$ be our set of wedges, such that any pair
of them is NC. Let $s'=f(s, 2)$.
Partition our point set $S$ into
$S'_1, S'_2, \ldots, S'_{t-1}$ such that
for $i=1, 2, \ldots , t-1$, for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S|\ge f(s', t-1)$ then
$|W'_i\cap S'_i|\ge s'=f(s, 2)$.
For each $i=1, 2, \ldots , t-1$, partition
$S'_i$ into two parts, $S''_i$ and $S^t_i$,
such that for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S'_i|\ge f(s, 2)$ then
$|W'_i\cap S''_i|\ge s$, and
for any translate $W'_t$ of $W_t$,
if $|W'_t\cap S'_i|\ge f(s, 2)$ then
$|W'_t\cap S^t_i|\ge s$.
Finally,
for $i=1, 2, \ldots , t-1$, let $S_i=S''_i$ and
let $S_t=\cup_{j=1}^{t-1}S^t_j$.
For $i=1, 2, \ldots , t-1$,
any translate $W'_i$ of $W_i$, if
$|W'_i\cap S|\ge f(s', t-1)$ then
$|W'_i\cap S'_i|\ge s'=f(s, 2)$, so
$|W'_i\cap S_i|\ge s$,

And for any translate $W'_t$ of $W_t$, if
$|W'_i\cap S|\ge f(s', t-1)$,
then for some $i=1, 2, \ldots t-1$,
$|W'_t\cap S'_i|\ge \frac{f(s', t-1)}{t-1}\ge f(s,2)$, therefore,
$|W'_t\cap S^t_i|\ge s$, so
$|W'_t\cap S_t|\ge s$.
This concludes the proof of Lemma 7. \hfill $\Box$

\smallskip

\noindent {\bf Remark.} The proofs of Lemmas 2, 4, 5, and 6 imply that
$f(1, 2)\le 8$. Combining it with the proof of Lemma 7 we get the bound
$f(s,t)\le (8s)^{2^{t-1}}$.

As a corollary, we have proved Lemma \ref{sokwedge}.
\medskip

\noindent {\bf Lemma \ref{sokwedge}.} {\em A set of wedges ${\cal W}=\{ W_1, W_2, \ldots ,
W_t \}$ is NC if and only if any pair $\{W_i, W_j \}$ is NC.}

\smallskip

\noindent {\bf Proof of Lemma \ref{sokwedge}.}
Clearly, if some pair $\{W_i, W_j \}$ is {\em not} NC, then the whole set
$\cal W$ is not NC either.
Suppose that every pair $\{W_i, W_j \}$ is NC.
Decompose $S$ into $t$ parts $S_1, S_2, \ldots , S_t$
with the property that
for $i=1, 2, \ldots , t$, for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S|\ge f(3, t)$ then
$|W'_i\cap S_i|\ge 3$.
Then, by Lemma \ref{1wedge}, each $S_i$ can be colored with red and blue such
that if
$|W'_i\cap S_i|\ge 3$
then $W'_i$ contains points of both colors.
So this coloring of $S$ has the property that
for $i=1, 2, \ldots , t$, for any translate $W'_i$ of $W_i$,
if $|W'_i\cap S|\ge f(3, t)$ then it contains points of both colors. \hfill $\Box$

\subsection{Summary of Proof of Theorem 1.}
Although we have already established Theorem 1, we find it useful to give another summary of the complete proof.

Suppose that $P$ is an open convex polygon of $n$ vertices and
${\cal P}=\{\ P_i\ |\ i\in I\ \}$ is a collection of translates of
$P$ which forms an
$M$-fold covering of the plane.
We will set the value of $M$ later.
Let $m$ be the minimum distance
between any vertex and non-adjacent side of $P$.
Take a square grid $\cal G$ of basic distance $m/2$.
Obviously, any translate of $P$ intersects at most
$K=4\pi(diam(P)+m)^2/m^2$ basic squares.
For each (closed) basic square $B$, using its compactness,
we can find a {\em finite} subcollection of the translates such that
they still form an $M$-fold covering of $B$.
Take the union of all these subcollections.
We have a {\em locally finite} $M$-fold covering of the plane.
That is, every compact set is intersected by finitely many of the translates.
It is sufficient to decompose this covering.
For simplicity, use the same notation
${\cal P}=\{\ P_i\ |\ i\in I\ \}$ for this subcollection.

We formulate
and solve the problem in its dual
form.
Let $O_i$ be the center of gravity of $P_i$.
Since ${\cal P}$ is an $M$-fold covering of the plane,
every translate of $\bar{P}$, the reflection of $P$ through the
origin, contains at least $M$ points of the locally finite set
${\cal O}=\{\ O_i\ |\ i\in I\ \}$.

The collection ${\cal P}=\{\ P_i\ |\ i\in I\ \}$ can be decomposed into two
coverings
if and only if the set ${\cal O}=\{\ O_i\ |\ i\in I\ \}$ can be colored with
two colors, such that every translate of $\bar{P}$ contains a point of both
colors.

Let ${\cal W}=\{ W_1, W_2, \ldots , W_n \}$ be the set of wedges
that correspond to the vertices of $\bar{P}$.
By the convexity of $\bar{P}$,
no pair $\{W_i, W_j \}$ is of Type 5 (Special), therefore,
by the previous Lemmas,
each pair is NC. Consequently, by Lemma 8, ${\cal W}$ is
NC as well. So there is a $k$ with the following property.

\smallskip

\noindent {\bf *}  Any set of points $S$ can be colored with two colors such that
any translate of $W_1, W_2, \ldots , W_n$
that contains at least $k$ points of $S$, contains points of both colors.

\smallskip

Choose $M$ such that $M\ge kK$, and color the points of
$\cal O$ in each basic square separately, with property {\bf *}.

Since any translate $P'$ of $\bar{P}$ intersects at most
%$40A(P)/m^2$
$K$ basic squares of the grid $\cal G$, $P'$ contains at least $M/K\ge k$ points of
${\cal O}$ in the same basic square $B'$.
By the choice of the grid $\cal G$,
$B'$ contains at most one vertex of $P'$, hence
$B'\cap P'=B'\cap W$, where $W$ is a translate
of some $W_i\in {\cal W}$. So, by property {\bf *},
$P'$ contains points of ${\cal O}\cap B'$ of both colors.
This concludes the proof of Theorem 1. \hfill $\Box$

\subsection{Concluding Remarks}
Throughout this paper we made no attempt to optimize the constants.
However, it may be 
an
interesting problem to determine (asymptotically) 
the smallest $k$ in the proof of
Theorem 1. 

Another interesting question is to decide whether
this constant depends only on the number of vertices of the polygon or on the
shape as well. In particular, we cannot verify the following.

\medskip

\noindent {\bf Conjecture.} {\em There is a constant $k$ such that any
$k$-fold covering of the plane with translates of a
convex quadrilateral
can be decomposed into two coverings.}

\medskip

One can also investigate whether a given covering can be decomposed into
$s$ coverings, for some fixed $s$. 
For any planar set $P$ and $s\ge 1$, if it exists, 
let $k=k(s, P)$ be the smallest 
number such that any $k$-fold covering of the plane with translates of
$P$ can be decomposed into $s$ coverings. 
By Theorem 1, $k(2, P)$ exists for any open convex polygon $P$.
With a slight modification 
of its proof, we get the following more general result.

\medskip

\noindent {\bf Theorem 1'.} {\em For any open convex polygon $P$, and any 
$s$, there exists a (smallest) number $k=k(s, P)$ such that 
any $k$-fold covering of the plane with translates of
$P$ can be decomposed into $s$ coverings. }

\medskip

Our proof gives $k(s, P)<K_P(8s)^{2^{n-1}}$, where $K_P$ is the constant $K$ from the
proof of Theorem 1 and $n$ is the number of vertices of $P$. 
For {\em centrally symmetric} open convex polygons 
Pach and T\'oth \cite{PT07} established 
a much better upper bound, 
which is quadratic in 
$s$.
Recently, 
Aloupis et al. \cite{A08} improved it to linear. 
They showed that, for any centrally symmetric open convex polygon
$P$, there is an $\alpha_P$ such that
$k(s, P)<\alpha_Ps$.
The best known lower bound on $k(s, P)$ is $(s, P)\ge\lfloor 4s/3\rfloor-1$
\cite{PT07}.
 
\medskip

Our proofs use the assumption that the covering is locally finite, and 
for open polygons we 
could find a locally finite subcollection which is still a $k$-fold covering.
Still, we strongly believe that Theorem 1 holds for closed convex polygons
as well.

\medskip

\noindent {\bf Acknowledgement.} We are very grateful to the anonymous
referee
for his remarks.





==> frontold.tex <==

\begin{center}
{\fontsize{17}{0}\textbf{Decomposition of Geometric Set Systems and Graphs % \\[0pt]
}}
\vspace{10mm}

{\Large \ \textsc{PhD Thesis} }
\end{center}

{\large \vspace{10mm} }

\begin{center}
{\Large \textsc{ Written by:} \; Pálvölgyi Dömötör }

{\large \vspace{5mm} }

{\Large \textsc{ Supervisor:} \; Pach János }
\end{center}

{\large \vspace{10mm} }

\vskip 5cm
{\large
\begin{figure}[th]
\begin{center}
{\large \epsfig{file=epfllogo.eps,angle=0,width=0.2\textwidth}  }
\end{center}
\end{figure}
}


\begin{center}
{\large \vspace{10mm} }
%{\large Ecole Polytechnique Federale de Lausanne }

{\large Facult\'e des Sciences de Base \\}

{\large 2010 }

\end{center}

==> org.tex <==

I would like to thank

%elte, epfl, esp keszegh, katona, kiraly, geza, jani

%padmini, family
